Zero-Shot Feature Selection via Transferring Supervised Knowledge

Feature selection, an effective technique for dimensionality reduction, plays an important role in many machine learning systems. Supervised knowledge can significantly improve the performance. However, faced with the rapid growth of newly emerging concepts, existing supervised methods might easily suffer from the scarcity and validity of labeled data for training. In this paper, the authors study the problem of zero-shot feature selection (i.e., building a feature selection model that generalizes well to "unseen" concepts with limited training data of "seen" concepts). Specifically, they adopt class-semantic descriptions (i.e., attributes) as supervision for feature selection, so as to utilize the supervised knowledge transferred from the seen concepts. For more reliable discriminative features, they further propose the center-characteristic loss which encourages the selected features to capture the central characteristics of seen concepts. Extensive experiments conducted on various real-world datasets demonstrate the effectiveness of the method.

==> abstract_ijca.tex <==
\begin{abstract}
%Feature selection has shown its efficiency in facilitating high-dimensional data.
%Feature selection plays an important role in pattern recognition and image processing systems.
%Feature selection (FS) has been widely utilized in pattern recognition systems.
Feature selection plays an important role in pattern recognition systems.
%Supervised knowledge is capable of significantly improving the quality of selected features.
%Supervised knowledge is capable of significantly improving the FS performance.
Supervised knowledge can significantly improve the performance.
% quality of selected features.
%Despite this importance, existing work fail to xxxxxxx.
However, confronted with the rapid growth of newly-emerging concepts, existing supervised methods may easily suffer from the scarcity of labeled data for training.
%However, new concepts and multimedia data emerge every day, making collecting supervised information for re-training feature selection model infeasible.
%In this paper, we study the problem of \emph{Zero-Shot Feature Selection}, i.e., building a feature selection model that generalizes well to ``unseen'' concepts with limited training data of ``seen'' concepts.
Therefore, this paper studies the problem of \emph{Zero-Shot Feature Selection}, i.e., building a feature selection model that generalizes well to ``unseen'' concepts with limited training data of ``seen'' concepts.
%Therefore, this paper studies the \emph{Zero-Shot Feature Selection} problem, i.e., building a feature selection model that generalizes well to ``unseen'' concepts with limited training data of ``seen'' concepts.
%identifying key features for the coming unseen concepts with limited training data of seen concepts.
%(ZSFS)
%In this paper, we propose a novel feature selection scheme, termed \emph{Zero-Shot Feature Selection (ZSFS)}, which could select representative features for the images of ``unseen'' classes but only learn with the limited training data of ``seen'' classes.
%The goal is to select representative features for the images of ``unseen'' categories, which towards to images of ``unseen'' categories learned from limited training data of ``seen'' categories.
%Specifically, we project the original independent labels (i.e., 0/1-form label vectors) to semantic embedding space, so as to bridge the gap between seen and unseen categories.
%Specifically, we replace the original binary labels (i.e., 0/1-form label vectors) with semantic attribute vectors which provide discriminative properties of unseen categories.
%Specifically, to transfer the supervised knowledge to the coming unseen classes, we replace the original labels with semantic attribute labels.
%Specifically, to transfer knowledge from seen concepts to unseen concepts, in the seen area, we propose to replace the original class labels with attribute descriptions.
%Specifically, motivated by zero-shot learning, we adopt the semantic vectors of concepts to capture the discriminant structure among classes, making the model trained with seen concepts generalize well for unseen ones.
%To address this problem, inspired by zero-shot learning, we adopt class-semantic descriptions as supervision knowledge for FS model.
To address this, inspired by zero-shot learning, we use class-semantic descriptions which provide additional semantic information about unseen concepts as supervision.
%in the seen area,
%propose to train FS model with class-semantic descriptions.
%, making the model trained with seen concepts generalize well for unseen ones.
%we use semantic attribute labels to replace the original labels.
%(i.e., 0/1-form label vectors)
%Since these attributes provide semantic information about the unseen categories, as such, the selected features could xxxx.
%Since these attributes provide the discriminative semantic properties about the unseen categories, the selected features could xxxx.
%Then the features, which best generates these semantic representations, are selected for the ``unseen'' categories.
%In addition, to seek for more reliable discriminative features, our method ensures the selected features lie in the center of seen categories.
%In addition, to seek for more reliable discriminative features, we propose another new loss function (i.e., \emph{center-characteristic loss}) to make the selected features capture the central characteristics of seen classes.
%In addition, to seek for more reliable discriminative features, we encourage the selected features to capture the central characteristics of seen classes and formulate this by a novel loss function (i.e., \emph{center-characteristic loss}).
In addition, to seek for more reliable discriminative features, we further propose a novel loss function (named \emph{center-characteristic loss}) which encourages the selected features to capture the central characteristics of seen concepts.
  %We further formulate this purpose by a novel loss function named center-characteristic loss.
%Finally, we develop an efficient alternating algorithm to solve the proposed ZSFS model.
Experimental results on three benchmarks demonstrate the superiority of the proposed method.
%Experimental results on three datasets demonstrate the superiority of our method.
%Extensive experimental results demonstrate the effectiveness of our method.
%Extensive experimental results demonstrate the superiority of our method.
\end{abstract} 

==> compared_method.tex <==
\section{Compared methods}
\begin{equation}
\label{eq_final_cost}
\begin{aligned}
& \underset{W}{\text{min}} & & \mathcal{J} = \left \| Y-XW \right \|^{2}_{F} + \gamma \left \| W \right \|_{21}
\end{aligned}
\end{equation}
where $W \in R^{n \times c}$ .
The L21-norm regularization term is imposed on $W$ to ensure that $W$ is sparse in rows, i.e., it achieves joint feature sparsity for all c latent semantic variables.

\begin{equation}
\label{eq_final_cost}
\begin{aligned}
& \underset{W}{\text{min}} & & \mathcal{J} = \left \| Y-XW \right \|^{2}_{F} + \gamma Tr(W^{T}DW)
\end{aligned}
\end{equation}
where $D$ is a diagonal matrix with the $i$-th diagonal element as:
$$D(i,i) = \frac{1}{2\left \| W(i,:) \right \|_{2} }$$

The derivations of $\mathcal{J}$ w.r.t. $W$ are:
\begin{equation}
\label{eq_update}
\begin{aligned}
&\frac{\partial \mathcal{J}}{\partial W} = -2X'Y + 2X'XW +2\gamma DW
\end{aligned}
\end{equation} 

==> experiments_ijcai.tex <==


\begin{figure*}[!t]
\centering
\subfigure[SUN]{
    \includegraphics[width=0.28\textwidth]{images/clustering/SUN_ACC}
}
\subfigure[aPY]{
    \includegraphics[width=0.24\textwidth]{images/clustering/aPY_ACC}
}
\subfigure[CIFAR10]{
    \label{fig:ACC_CIFAR10}
    \includegraphics[width=0.24\textwidth]{images/clustering/CIFAR10_ACC}
}
\caption{Clustering results (ACC).}
\label{fig_ACC}
\end{figure*}
%26 22 22
%27 23 23

\section{Experiments}\label{sect_expriment}
%In this section, we conduct extensive experiments to evaluate the performance of the proposed XXXXX for the task of feature selection.
%To show the effectiveness of our method, we compare our method to both states-of-the-art unsupervised and supervised feature selection methods.
%Leveraging related source domain for feature selection is so far an unexplored area.
%To the best of our knowledge, there is no directly related work to compare with.
%%Therefore, in this section, we compare our method to state-of-the-art unsupervised as well as supervised feature selection methods.
%For an extensive comparison, we compare our method CCFS to both state-of-the-art unsupervised and supervised feature selection methods.
%%Specifically, we compare with unsupervised methods in the task of clustering, and compare with supervised methods in the task of classification.
%%All the compared methods are directly applied on the target data so as to compare with ours.
%Since existing methods cannot address the cross-class case, we directly apply these compared methods on the target data so as to compare with ours.
%In this section, we present experimental details to verify the effectiveness of the proposed framework, CCFS.
%Firstly, we introduce three real-world datasets.
%Then, for an extensive comparison, we compare our method with unsupervised and supervised feature selection methods on the task of clustering and classification, respectively.
%Lastly, we study the convergence of the proposed optimization algorithm (Alg.~\ref{alg_ours}) and the effect of parameters on performance.
\begin{table}[!t]
%\scriptsize
\small
\caption{The statistics of datasets}
\centering % used for centering table
\begin{tabular}{l|rrr}
\hline
                   &SUN &aPY      &CIFAR10 \\
\hline
\hline
\# seen concepts           &707      &20       &2    \\
\# seen images            &14,140  &12,695     &12,000  \\
\# unseen concepts           &10      &12         &8 \\
\# unseen images            &200   &2,644      &48,000 \\
\# attributes                &102     &64         &50    \\
\# features                  &4,096  &4,096      &4,096 \\
\hline
\end{tabular}
\label{tab_dataset}
\end{table}
%\begin{table}[htbp]
%\caption{Datasets}
%\centering % used for centering table
%\begin{tabular}{l|rrr}
%\hline
%                   &SUN &aPY      &AwA \\
%\hline
%\hline
%\# source classes           &707      &20       &40    \\
%\# source images            &14,140  &12,695     &24,295  \\
%\# target classes           &10      &12         &10 \\
%\# target images            &200   &2,644      &6,180 \\
%\# attributes                &102     &64         &85    \\
%\# features                  &4,096  &4,096      &4,096 \\
%\hline
%\end{tabular}
%\label{tab_dataset}
%\end{table}
\subsection{Experimental Setup}


\paragraph{Datasets}
%We test our method on three benchmark datasets with attributes.
The experiments are conducted on three widely used datasets.
%: SUN scene attributes database (\textbf{SUN})~\cite{patterson2012sun}, aPascal/aYahoo objects dataset (\textbf{aPY})~\cite{farhadi2009describing} and \textbf{CIFAR10}~\cite{lampert2009learning}.
%The first dataset is SUN scene attributes database (\textbf{SUN})~\cite{patterson2012sun} which contains 14,340 images from 717 different scenes like ``village'' and ``airport''.
%The first dataset is \textbf{SUN}~\cite{patterson2012sun} which contains 14,340 images from 717 different scenes like ``village'' and ``airport''.
\textbf{SUN}~\cite{patterson2012sun} is the first dataset which contains 14,340 images from 717 different scenes like ``village'' and ``airport''.
%SUN scene attributes database (\textbf{SUN})~\footnote{https://cs.brown.edu/~gen/sunattributes.html}~\cite{patterson2012sun} is the first dataset which contains 14,340 images from 717 different scenes like ``village'' and ``airport''.
%Each image is annotated by a 102-dimensional binary attribute vector manually.
For each image, a 102-dimensional binary attribute vector is annotated manually.
We average the images' attributes to obtain the attributes for each concept, and follow the seen/unseen split setting as~\cite{jayaraman2014zero}.
%and we average.
%We obtain the attribute labels of each seen class by averaging attribute vectors of the instances belonging to that class.
%%For each image, 102-dimensional binary attributes are annotated manually.
%%%We average the image attributes to obtain the class attributes.
%%We obtain the attribute representation of each class by averaging attribute vectors of the instances belonging to that class.
%We follow the seen/unseen split setting in~\cite{jayaraman2014zero}.
%, and extract deep features using DeCAF~\cite{donahue2014decaf}.
%This dataset provides a standard source/target split where 40 classes are in the source domain and 10 classes are in the target domain.
%We use the recently provided DECAF features~\cite{donahue2014decaf} of this dataset.
%The second dataset is aPascal/aYahoo objects dataset (\textbf{aPY})~\cite{farhadi2009describing} which contains two subsets.
%aPascal/aYahoo objects dataset (\textbf{aPY})~\cite{farhadi2009describing}~\footnote{http://vision.cs.uiuc.edu/attributes/} is the second dataset which contains two subsets.

\textbf{aPY}~\cite{farhadi2009describing} is the second dataset which contains two subsets: aPascal and aYahoo.
The aPascal subset contains 20 different concepts from VOC2008 dataset.
The aYahoo subset has another 12 different categories collected by Yahoo image search engine.
%This dataset has a standard split setting, i.e., aPascal and aYahoo serve as the seen part and unseen part respectively.
%aPascal/aYahoo objects dataset (\textbf{aPY})~\cite{farhadi2009describing} is the second dataset which contains two subsets.
%\textbf{aPY}~\cite{farhadi2009describing} is the second dataset which contains two subsets.
%The aPascal subset comes from PASCAL VOC2008 dataset, and contains 20 different concepts, such as ``people'' and ``dog''.
%The aYahoo subset is collected by Yahoo image search engine, and has 12 similar but different categories compared to aPascal, such as ``monkey'' and ``zebra''.
This dataset has a standard split setting, i.e., aPascal and aYahoo serve as the seen part and unseen part respectively.
%In this dataset, each image is annotated by a 64-dimensional binary attribute vector, such as “furry” and “pot”.
%We follow its standard split setting where the PASCAL part and Yahoo part serves as the seen part and unseen part respectively.
%We follow the standard setting where the PASCAL part and Yahoo part serves as the source and target domain respectively.
%The PASCAL part serves as source domain, and the Yahoo part as target domain.
Each image is annotated by a 64-dimensional binary attribute vector.
%We average the images’ attributes to obtain the attribute labels for each seen class.
%We get the attribute labels for each class by averaging the attribute vector of each image.
% is annotated by a 64-dimensional binary attribute vector, and we average the images’ attributes to obtain the attribute labels for each class.
We average the attribute vectors of images in the same category to get the class attribute description.
%We use the author-provided features, such as SIFT and color histograms.
%We use the provided 9,751-dimensional ``hand-crafted'' low-level features, such as SIFT and color histograms.
%\textbf{AwA} contains 30,475 images from 50 animal classes, and each class is described by a 85-dimensional binary attribute vector.
%We adopt its standard source/target split, and use the recently provided DeCAF features.
%The third dataset is \textbf{CIFAR10}~\cite{krizhevsky2009learning} which consists of 10 concepts of objects with 6,000 images per concept.

\textbf{CIFAR10}~\cite{krizhevsky2009learning} is the third dataset which consists of 10 classes of objects with 6,000 images per class.
%and each class has 6,000 images.
%Since this dataset does not have a standard seen/unseen split setting, we simply use the first two classes (i.e., ``airplane'' and ``automobile'') as seen classes and use the others as unseen classes.
Since this dataset does not have a standard seen/unseen split setting, we randomly adopt two concepts as seen.
Thus, we have $C_{10}^{2}$ different seen/unseen splits.
%Compared to the above two datasets, the split of CIFAR10 shows another extreme setting where most of the classes are unseen.
%The purpose of this setting is to test the extreme case where most of the concepts are unseen.
In addition, as this dataset does not have any attribute annotations, we adopt the 50-dimensional word vector provided by~\cite{huang2012improving} as attribute label for each concept.
%, i.e., these attributes are automatically generated.
Concretely, these embedding vectors are automatically generated from a Wikipedia corpus~\cite{shaoul2010westbury} with a total of about 2 million articles and 990 million tokens.
%use the tool provided by~\cite{huang2012improving} to 50-dimensional word vector for each of as attribute labels.
%adopt the 50-dimensional word vector provided by as

For all these three datasets, we use the widely used 4,096-dimensional deep features provided by~\cite{guo2016semi}.
%the 4,096-dimensional features provided by~\cite{guo2016semi}.
%Specifically, the features of each image are extracted by the pre-trained Deep CNN tool Caffe~\cite{donahue2014decaf}.
The detailed statistics of these three benchmarks are listed in Table~\ref{tab_dataset}.
%Table~\ref{tab_dataset} lists the detailed statistics of these datasets.

%For all these three datasets, we utilize the pre-trained Deep CNN tool Caffe~\cite{donahue2014decaf} and use the output of the fc7 layer which yields a 4,096-dimensional vector for each image.

%This dataset provides a standard source/target split where 40 classes are in the source domain and 10 classes are in the target domain.
%We use the recently provided DECAF features~\cite{donahue2014decaf} of this dataset.


%The classical \emph{K}-means clustering is
%The selected features by different methods
%------------------
%%use the clustering performance to evaluate the quality of selected features.
%%Two commonly used clustering quality evaluation metrics, [4] are used in our experiment.
%With the selected features, we evaluate the performance in terms of \emph{K}-means clustering by two widely used metrics, i.e., Accuracy (ACC) and Normalized Mutual Information(NMI).
%Since \emph{K}-means clustering is sensitive to initialization, we repeat the clustering 20 times with random initialization and report the results corresponding to best objective function values.
%
%Each feature selection algorithm is first performed to select features, then K-means clustering is performed based on the selected fea-tures. Since K-means often converges to local minima, we repeat each experiment 20 times and report the average performance.


%  record the average results.
\paragraph{Comparison methods}
We compare the proposed method \myalg\ with both unsupervised and supervised FS methods:
%On one hand, we test the proposed method ZSFS.
%ZSFS$\backslash$\emph{scl}
%we test the ZSFS$\backslash$scl - Eliminating the effect of self-center loss by setting $\alpha = 0$.
%ZSFS$_{Eq.1}$ can be seen as the classical Lasso problem with the modified supervised knowledge.
%Besides, we also test the (i.e., $\alpha=1$ in ZSFS), which can be seen as the classical Lasso problem with the modified supervised knowledge.
%Since this is the first study to handle the Zero-Shot Feature selection problem, we compare our methods with state-of-the-art unsupervised and supervised feature selection methods:
%In summary, we compare our two methods with the following state-of-the-art unsupervised and supervised feature selection methods:
%we test the ZSFS$\backslash$scl - Eliminating the effect of self-center loss by setting $\alpha = 0$.
%\textbf{ZSFS$_{Eq.1}$} can be seen as the classical Lasso problem with the modified supervised knowledge.
%Besides, we also test the (i.e., $\alpha=1$ in ZSFS), which can be seen as the classical Lasso problem with the modified supervised knowledge.
%We compare these two versions of method with state-of-the-art unsupervised and supervised feature selection methods:
%In summary, we compare ours to the following methods:
\begin{enumerate}\setlength{\itemsep}{-0.0cm}
  \item Random method selects features randomly.
  %which evaluates features according to their ability of preserving the local manifold structure.
  \item MCFS~\cite{cai2010unsupervised} is an unsupervised method selecting features by using spectral regression with $\ell_{1}$-norm regularization.
%  \item TRACK~\cite{wang2014unsupervised} which selects features via a unified trace ratio formulation and \emph{K}-means clustering.
  %\item RUFS, which performs robust clustering and ro-bust feature selection simultaneously to select the most important and discriminative features.
  \item FSASL~\cite{du2015unsupervised} is an unsupervised method performing structure learning and feature selection simultaneously.
  %\item LASSO~\cite{tibshirani1996regression} is the classical supervised feature selection method (we adopt $\ell_{2,1}$-norm regularization~\cite{nie2010efficient} for computation efficiency).
  \item LASSO~\cite{tibshirani1996regression} is the classical supervised FS method.
  \item L20ALM~\cite{cai2013exact} is a supervised method evaluating features under an $\ell_{21}$-norm loss function with $\ell_{20}$-norm constraint.
  \item CSFS~\cite{liu2017cost} is a newest supervised method considering the class imbalance problem of labeled data.
\end{enumerate}
In addition, to validate the effectiveness of the proposed center-characteristic loss, we test a variant of our method (denoted as \emph{\myalgv}) by setting $\alpha {=} 0$ in Eq.~\ref{eq_final_cost_relax} to eliminate the effect of this loss term.
Another point to be noted is that we apply all methods on seen concepts and then evaluate the quality of selected features on unseen concepts.
In other words, in the training phase, the unseen concepts are invisible to all methods.

\begin{figure*}[t]
\centering
\subfigure[SUN]{
    \includegraphics[width=0.28\textwidth]{images/clustering/SUN_NMI}
}
\subfigure[aPY]{
    \includegraphics[width=0.24\textwidth]{images/clustering/aPY_NMI}
}
\subfigure[CIFAR10]{
    \label{fig:NMI_CIFAR10}
    \includegraphics[width=0.24\textwidth]{images/clustering/CIFAR10_NMI}
}
\caption{Clustering results (NMI).}
\label{fig_NMI}
\end{figure*}

\paragraph{Experimental Setting}
Since determining the optimal number of selected features is still an open problem~\cite{tang2012unsupervised}, we follow~\cite{du2015unsupervised} to vary the selected features number from 5 to 50 in intervals of 5.
%Similar to~\cite{du2015unsupervised}, the number of selected features varies from 5 to 50 in intervals of 5.
% ranges from 1 to 10 with incremental step 1
%With the selected features, we evaluate the performance in terms of \emph{K}-means clustering by two widely used metrics, i.e., Accuracy (ACC) and Normalized Mutual Information (NMI)~\cite{duda2012pattern}.
%As the unseen concepts have no labeled data, we follow the common way to evaluate unsupervised feature selection, i.e., evaluating the selected feature on clustering task.
%As the unseen concepts have no labeled data, we follow the common way to evaluate unsupervised feature selection on the clustering task~\cite{cai2010unsupervised}.
As the unseen concepts have no labeled data, we evaluate the selected features on the clustering task, so as to follow the current practice of evaluating unsupervised FS methods~\cite{cai2010unsupervised}.
%which is the most common way for unsupervised feature selection evaluation~\cite{cai2010unsupervised}.
%which is the common way for unsupervised feature selection evaluation.
%we follow the common way to evaluate unsupervised feature selection on the clustering task~\cite{cai2010unsupervised}.
%Following the common way to evaluate unsupervised feature selection, we evaluate the selected feature on clustering task.
%evaluate the quality of
%follow the common way to evaluate unsupervised feature selection
%we evaluate the quality of selected features is valuated in terms of clustering performance.
Specifically, we employ the classical \emph{K}-means clustering method and adopt two widely used clustering metrics, i.e., Accuracy (ACC) and Normalized Mutual Information (NMI)~\cite{duda2012pattern}.
%The quality of selected features is valuated in terms of \emph{K}-means clustering performance by two widely used metrics, i.e., Accuracy (ACC) and Normalized Mutual Information (NMI)\footnote{www.cad.zju.edu.cn /home/dengcai/Data/Clustering.html}~\cite{duda2012pattern}.
%We evaluate the in terms of clustering performance.
%Two widely used clustering quality evaluation metrics, Accuracy (ACC) and Normalized Mutual Information (NMI)~\cite{duda2012pattern}, are used.
%We perform \emph{K}-means to cluster target images with the selected features.
Since \emph{K}-means is sensitive to initialization, we repeat the clustering 20 times with random initializations and report the average performance.
%To tune the parameters of all methods, we carry out 5-fold cross-validation on the seen classes, i.e., training on four folds of seen data and testing on the remaining single fold.
%Specifically, we create the validation set by grouping all instances belonging to 20\% of the seen classes chosen at random (without replacement).
%Specifically, we train different methods on four folds of the seen data, and test on the remaining single fold.
% chosen at random (without replacement).
%All parameters are tuned by grid search with $\{10^{-2},10^{-1},10^{0},10^{1},10^{2}\}$.
%from the grid by a “grid-search” strategy from
%Besides, to tune the parameters of all methods, we carry out cross-validation on the seen classes for all methods.
%%, and turn all parameters by a ``grid-search'' strategy from $\{10^{-2},10^{-1},10^{0},10^{1},10^{2}\}$.
%In the compared methods, all parameters are tuned by a ``grid-search'' strategy from $\{10^{-2},10^{-1},10^{0},10^{1},10^{2}\}$.
%In our methods, parameters are selected from the same ``grid'' via cross-validation on the seen concepts.
Besides, the parameters of all methods are tuned by a ``grid-search'' strategy from $\{10^{-2},10^{-1},10^{0},10^{1},10^{2}\}$ based on cross-validation on the seen concepts.

%The parameters of all methods are set by 5-fold cross validation using the seen data, i.e., training on four folds and testing on the remaining single fold.
%%Specifically, we train
%All parameters are tuned by grid search with $\{10^{-2},10^{-1},10^{0},10^{1},10^{2}\}$.



\subsection{Clustering with Selected Features}
Figure~\ref{fig_ACC} and Figure~\ref{fig_NMI} show the clustering performance in terms of ACC and NMI, respectively.
There are several important observations here.
Firstly, our methods (both \myalg\ and \myalgv) always outperform the others significantly, in terms of both ACC and NMI, on all datasets.
For example, with 20 selected features, our two methods outperform the best baseline by 20–-40\% relatively in terms of ACC.
The underlying principle is that our methods successfully deduce the knowledge of unseen concepts by introducing attributes.

Secondly, it is interesting to find that the unsupervised method MCFS is comparable to or even better than those supervised baselines.
%An interesting observation is that the unsupervised method MCFS gains competitive even better performance than the supervised method L20ALM.
This indicates that the supervised methods may be misled by the seen concept labels which provide little information about unseen concepts.
Intuitively, we can understand this by the fact that old knowledge may often need to be modified to fit the new problem.
      %Another interesting observation is t

Thirdly, on the CIFAR10 dataset where most concepts are unseen and attributes are automatically generated, our methods could still identify high quality features (Figs.~\ref{fig:ACC_CIFAR10} and~\ref{fig:NMI_CIFAR10}).
This confirms the flexibility of our methods as well as the advantage of attributes.
Lastly, \myalg\ consistently obtains more stable and better performance than \myalgv.
This phenomenon indicates that the proposed center-characteristic loss can help to select reliable discriminative features for unseen concepts with limited labeled seen instances.


%\begin{itemize}\setlength{\itemsep}{0cm}
%  \item Our methods (both \myalg\ and \myalgv) always outperform the others significantly, in terms of both ACC and NMI, on all datasets.
%  For example, with 20 selected features, our two methods outperform the best baseline by 20–-40\% relatively in terms of ACC.
%The underlying principle is that our methods successfully transfer the supervised knowledge to unseen concepts by introducing attributes.
%  \item An interesting observation is that the unsupervised method MCFS is comparable to or even better than those supervised baselines.
%  %An interesting observation is that the unsupervised method MCFS gains competitive even better performance than the supervised method L20ALM.
%  This indicates that the supervised methods may be misled by the seen concept labels which provide little information about unseen concepts.
%      %Another interesting observation is t
%  \item On the CIFAR10 dataset where most concepts are unseen and attributes are automatically generated, our methods could still identify high quality features (Figs.~\ref{fig:ACC_CIFAR10} and~\ref{fig:NMI_CIFAR10}).
%This confirms the flexibility of our methods as well as the advantage of attributes.
%  \item \myalg\ consistently obtains more stable and better performance than \myalgv.
%This phenomenon indicates that the proposed center-characteristic loss can help to select reliable discriminative features for unseen concepts with limited labeled seen instances.
%\end{itemize}
%
%1) Our methods (both ZSFS and ZSFS$_{Eq.1}$) always outperform others significantly, in terms of both ACC and NMI, on all datasets.
%The underlying principle is that our methods successfully transfer the supervised knowledge to the unseen classes by introducing attribute labels.
%2) Another interesting observation is the performance of unsupervised method MCFS gains competitive even better results than the supervised method L20ALM.
%This indicates that the supervised methods may be misled by the class labels which provide little information about the unseen classes.
% %to the training data of seen classes.
%3) On the CIFAR10 dataset where most classes are unseen and attributes are automatically generated, our methods could still identify high quality features (Figs.~\ref{fig:ACC_CIFAR10} and~\ref{fig:NMI_CIFAR10}).
%%they are a few seen classes as well as large test unseen classes
%This demonstrates the flexibility of our methods as well as the advantage of attribute labels.
%4) ZSFS consistently obtains more stable and better performance than ZSFS$_{Eq.1}$.
%This phenomenon indicates that the proposed center-characteristic loss can help to select reliable discriminative features for the unseen classes with limited labeled seen instances.

%%There are two important observations here.
%The first observation is that our methods (both ZSFS and ZSFS$_{Eq.1}$) always outperform others significantly, in terms of both ACC and NMI, on all datasets.
%%For instance, ZSFS outperforms the best comparative method by almost xxx on xx dataset.
%%The major reason may be that our methods reuse the supervised knowledge in seen classes through introducing the attribute labels of seen classes.
%The underlying principle is that our methods successfully transfer the supervised knowledge to the unseen classes by introducing attribute labels to the training data of seen classes.
%%In contrary, all the compared methods, which fail to transfer knowledge from seen classes, perform significantly worse than ours.
%%the compared method LASSO, which also uses pseudo labels but ignores cross-class knowledge,
%%This indicates that the proposed method is an effective framework for selecting high-quality features for the unseen classes.
%Another interesting observation is the performance of unsupervised method MCFS gains competitive even better results than the supervised method L20ALM.
%This indicates that the supervised method may be misled by the original labels which provide little useful information about the unseen classes.
%%, since the task is to distinguish unseen data.
%The last observation is that ZSFS consistently obtains more stable and better performance than ZSFS$_{Eq.1}$.
%%Specifically, ZSFS could get more stable performance.
%This phenomenon indicates that the proposed center-characteristic loss can enhance to select reliable discriminative features for the unseen classes with limited labeled seen instances.
%%3) The last observation is that xxx. It is worthy to note that our methods enjoys higher performance only with 5 features, which is preferred by the real-world applications to achieve satisfactory results with as few as features.
%%Our method are effective in the special situations.
%%In regions with less features(xxx), our method xxx. In regions with more features, our method xxx.
%%An interesting observation is the performance of MCFS, which is an unsupervised method, gains competitive even better results as compared to the supervised method L20ALM.



%\subsection{Optimization Effectiveness Analysis}
%We inspect the optimization algorithm for training \myalg.
%Figure~\ref{fig_iter_acc} shows the averaged clustering performance and objective function value w.r.t. each iteration in Alg.~\ref{alg_ours}.
%It can be observed that the objective function value decreases steadily with more iterations.
%Meanwhile, the classification performance increases and quickly reaches the highest accuracy in less than 20 steps.


\begin{figure}[!t]
\centering
\subfigure{
    \includegraphics[width=0.22\textwidth]{images/rate/SUN_ACC}
}
\subfigure{
    \includegraphics[width=0.22\textwidth]{images/rate/SUN_NMI}
}
\caption{Average clustering performance w.r.t. different labeled ratios of seen concepts on SUN.}
\label{fig_effect_ratio}
\end{figure}


\subsection{Effect of Labeled Seen Concept Ratio}
In this part, we evaluate the performance of the proposed method \myalg\ w.r.t. the labeled ratio in all seen concepts.
Specifically, in our method, we vary the labeled ratio of each seen concept from 0.1 to 1.
%keep the unseen class number unchanged and vary the labeled ratio of seen categories from 0.1 to 0.9.
%For simplicity, we experimentally set the parameters in our method as: $alpha=1$ and $\gamma=1$.
Figure~\ref{fig_effect_ratio} shows the average clustering performance on SUN (due to space limitations, we do not report the results on the other datasets, because we have similar observations on them).
It can be observed that even with only 10\% of seen concepts, \myalg\ could still benefit the success of cross-concept knowledge generalization.
This verifies the superiority of attributes for the ZSFS problem.
%This is consistent with the previous finding
On the other hand, as labeled ratio of seen concepts increases, our method shows an increasing advantage over the previous studies.
We analyse that with more seen concepts, \myalg\ would deduce more reliable supervision for the unseen concepts, thereby simultaneously improving the quality of selected features.

%have higher possibility to find relevant supervision for the unseen class,
%We analyse that with more seen concepts, \myalg\ can learn more reliable knowledge about the relationship between features and attributes, thereby simultaneously improving the quality of selected features.

%\subsection{Effectiveness of Semantic Attribute Labels}
\subsection{Advantage of Attribute Labels}
%\subsubsection*{Advantage}
%To further show the advantage of attribute labels, we use three methods: \myalg, \myalgv\ and the comparison method LASSO.
To further show the advantage of attributes, we use three methods: \myalg, \myalgv\ and the compared classical FS method LASSO.
%To further show the advantage of attribute labels, we use our methods (ZSFS and ZSFS$_{Eq.1}$) and the comparison method LASSO.
%We use three methods, ZSFS, ZSFS$_{Eq.1}$ and the compared method LASSO, for this purpose.
%We compare the effects of embedded labels and binary labels on three methods: ZSFS, ZSFS$_{Eq.1}$ and the compared method LASSO.
For clarity, we use $\mathcal{M}_{o}$ and $\mathcal{M}_{s}$ to denote the method $\mathcal{M}$ using the original class labels (i.e., $Y$) and semantic attributes (i.e., $Y_{s}$), respectively.
Figure~\ref{fig_semantic_compare} shows the averaged clustering results in terms of ACC.
It can be clearly observed that: compared to the original class labels, attributes could significantly improve the generalization ability of these FS methods.
%the performance of attribute labels is obviously better than that of class labels.
%As we can seen the performance of attribute labels is obviously better than that of class labels.
%In addition, even though only replacing binary labels with semantic labels for LASSO, we can obtain more than 10\% performance improvement.
The underlying reason is that attributes contain discriminative information about unseen concepts.
In contrast, the original class labels neglect this kind of knowledge, thereby leading to poor performance.
%Another interesting observation is that when switching to semantic labels, LASSO immediately obtains .

%\subsection{Limitation of Attribute Labels}
%%\subsubsection*{Limitation}
%%As pointed out, the success of our method relies on the used attributes which provide discriminative descriptions of unseen classes.
%Our method would fail in the case where the provided attributes cannot capture the discriminative properties shared between both seen and unseen classes.
%%seen classes and unseen classes have little attributes in common.
%This mainly occurs when the seen part and unseen part come from two different application scenarios, e.g., the scene dataset SUN and object dataset aPY are used as the seen and unseen parts respectively (we omit to report this result due to space limitations).
%%For example, the scene dataset SUN  and animal dataset aPY are adopted as the seen and unseen part respectively (we omit to report this result due to space limitations).
%%We omit this result due to space limitations.
%%How to select a reasonable seen class set for the coming unseen object may be a
%Intuitively, this problem can be solved by choosing appropriate seen classes for the specific application scenario, which we leave as our further work.

\begin{figure}[!t]
\centering
    %\includegraphics[width=0.30\textwidth]{images/semantic}
    \includegraphics[width=0.37\textwidth]{images/semantic}
%\caption{Averaged clustering accuracy: class labels vs. attributes.}
\caption{Average ACC: class labels vs. attributes.}
\label{fig_semantic_compare}
\end{figure}
%Selecting reasonable seen classes for the coming unseen object may be a
%Future works
%we use the scene dataset SUN as the seen classes, and the animal dataset aPY as the unseen classes (we omit this result due to space limitations).
%The above experiments validate this xxx on three datasets where the seen part and unseen part share some attributes.
%
%

%thereby leading to poor performance.

%
%To verify the effectiveness of semantic attribute labels, we compare three methods: ZSFS, ZSFS$_{Eq.1}$ and LASSO.
%Specifically,
%. We compare the effects of semantic labels and original binary labels for the following methods:

%The compared Lasso method (i.e., $\underset{W}{\text{min}} \mathcal{J} = \left \| Y_{s}-XW \right \|^{2}_{F} + \gamma \left \| W \right \|_{21}$)
%The compared Lasso method (i.e., $\underset{W}{\text{min}} \mathcal{J} = \left \| Y_{s}-XW \right \|^{2}_{F} + \gamma \left \| W \right \|_{21}$)
%\begin{table}[tpbh]
%\caption{The drop/decline when Semantic Embedding to independent labels}
%\centering % used for centering table
%\begin{tabular}{|l|r|r|r|}
%\hline
%                   &SUN &aPY      &AwA \\
%\hline
%\hline
%ACC           &-x      &-x      &-x    \\
%NMI            &-x  &-x     &-x  \\
%\hline
%\end{tabular}
%\label{tab_semantic}
%\end{table}

%\subsection{Effectiveness of Self-center Loss}
%1 When we switch the semantic embedding to binary labels, the results of self-center loss vs. classical L1 lasso.
%2 When center loss is replaced with original center loss, the result V.S..

%\begin{table}[tpbh]
%\caption{The xxxxxxx}
%\centering % used for centering table
%\begin{tabular}{|l|r|r|r|}
%\hline
%                   &SUN &aPY      &AwA \\
%\hline
%\hline
%ACC           &-x      &-x      &-x    \\
%NMI            &-x  &-x     &-x  \\
%\hline
%\end{tabular}
%\label{tab_center-loss}
%\end{table}


\begin{figure}[t]
\centering
\subfigure{
    \includegraphics[width=0.22\textwidth]{images/para/micro_alpha}
}
\subfigure{
    \includegraphics[width=0.22\textwidth]{images/para/macro_alpha}
}
\caption{The effect of parameter $\alpha$ on SUN.}
\label{fig_para}
\end{figure}

\subsection{Parameter Sensitivity}
In the proposed method \myalg, there is an important parameter $\alpha$ which controls the penalty of center loss.
% the contributions of xxx and xxx.
%controlling the contribution from label information.
%Figure~\ref{fig_para} shows the experimental results via changing the value of $\alpha$ (with the regularization parameter $\lambda{=}0.1$).
Figure~\ref{fig_para} shows the clustering performance w.r.t. this parameter on SUN (with the fixed regularization parameter $\lambda{=}1$).
It can be observed that our method is not very sensitive to $\alpha$, and the results remain almost the same when the parameters vary between $\{10^{-3}, ..., 10^{0} \}$ in our experiments.
%This empirically proves our convergence theory.



==> introduction_ijca.tex <==
\section{Introduction}
%In many real-world applications such as data mining and image processing, data are represented by high dimensional feature vectors.
%%Due to large amounts of data produced by rapid development of technology, the processing of high-dimensional data has become a big problem in many fields, such as computer vision, data mining, and pattern recognition.
%High dimensional data often contains quite a lot noise features, which are detrimental to practical applications.
%%As one of the typical method to alleviate this problem, feature selection attracts more and more attentions.
%%It aims to finding a subset of the most representative features from the original high-dimensional feature space.
%Feature selection~\cite{guyon2003introduction}, which aims to find a subset of the most representative features, has been proved to be one of the most important solutions to this problem.
The problem of feature selection (FS)~\cite{guyon2003introduction} has been widely investigated due to its importance for pattern recognition and image processing systems.
%saeys2007review
This problem can be formulated as follows: identify an optimal feature subset which provides the best trade-off between its size and performance for a given task.
%relevance
%The identified features not only provide an effective solution for the task, but also provide a dimensionally reduced base for understanding the underlying data~\cite{bicciato2003pca}.
%The identified features not only support an effective solution for the task, but also provide a more abstract view of the underlying data.
%a clearer
%a dimensionally-reduced view of the underlying data.
%~\cite{bicciato2003pca}.
%provide a effective insight into the relation of features and the task, to allow for a better understanding of the underlying data.
%represent a rational and dimensionally reduced base for understanding
%the basic biology of diseases
%The identified features provide an effective solution, provide insights into the relation of features and the task.
%The identified features can be seen an effective solution for the task, and can also be seen as a
%also provide insights into the features and their relation to the task and to allow for a better understanding of the underlying data

%for a given set of candidate features select the subset that provides the best tradeoff between its size and relevance for the given task.
%It aims to extract a small subset of feature from the problem domain while retaining a suitably high accuracy in representing the original features.
%The resulted subset can be seen as an effective solution for the task, and also provide insights into the features and their relation to the task.
%
%The selected features can provide insights into the features and their relation to the task, so as to allow for a better understanding of the underlying data.

%%~\cite{john1994irrelevant}
%Feature selection allows dimension reduction, which is crucial in reducing the noises of high-dimensional features.
%%reducing computational cost and storage space requirements.
%This is achieved by finding a subset of the most representative features from the original high-dimensional feature space.
%The resulted features not only maintains physical meaning of the original features and has better interpretability.
%As such, Compared to feature
%extraction, feature selection maintains physical meaning of the
%original features and has better interpretability.
%This is achieved by finding a subset of the most representative features from the high-dimensional feature setfor a compact and accurate data representation.
%find a subset of the most relevant features for a compact and accurate presentation of the original whole feature space.
%%Feature selection is an important problem for pattern recognition and image processing systems.
%%High-dimensional data is usually confronted in many real world applications, such as pattern recognition, computer vision, and data mining.
%It significantly increase the computational cost and storage space requirements.
%%Directly handling high-dimensional data not only significantly increases the time and space requirements,
%%Moreover, high-dimensional data may degenerate the performance of learning models, due to the curse of dimensionality~\cite{liu2007computational}.
%Moreover, high-dimensional data may lead to the incorrect data analysis results, due to the curse of dimensionality~\cite{liu2007computational}.
%%Curse of di-mensionality leads to great storage burden, high time com-plexity and failure of the classic learning machines
%%As one of the key method to alleviate this problem, feature selection  attracts substantial research attentions.
%%To solve this problem, feature selection techniques are designed to find a subset of the most representative features from the high-dimensional feature set for a compact and accurate data representation.
%Feature selection, which aims to find a subset of the most relevant features for a compact and accurate presentation, has been proved to be an effective way to fix this problem~\cite{john1994irrelevant,guyon2003introduction}.
%%
%Roughly, data-dependant hashing can be divided into two categories
%Existing feature selection methods can roughly be sub-divided into two categories: unsupervised and (semi-)supervised feature selection methods.
%%There are mainly two branches of feature selection methods, i.e., unsupervised and (semi-)supervised feature selection methods.
%%data-independent hashing and data-dependent hashing.
%Generally speaking, supervised methods~\cite{nie2010efficient,cai2013exact} usually achieve better performance than unsupervised ones.
%This is because supervised knowledge (e.g., labels or pair-wise relationships) can help to better explore the intrinsic properties of data.
%%data property.
%%Supervised knowledge (e.g., labels or pair-wise relationships) associated to data is capable of significantly improving the performance of feature selection methods.
%%Supervised knowledge (e.g., labels or pair-wise relationships) is capable of significantly improving the quality of selected features.
%% of feature selection methods.
%%In practice,


%Supervised knowledge (e.g., labels or pair-wise relationships) associated to data is capable of significantly improving the performance of FS methods~\cite{chandrashekar2014survey}.
%Supervised knowledge (e.g., labels or pair-wise relationships) associated to data is able to significantly improve the performance of FS methods~\cite{chandrashekar2014survey}.
Supervised knowledge (e.g., labels or pair-wise relationships) can significantly improve the quality of selected features~\cite{chandrashekar2014survey}.
%the performance of FS methods~\cite{chandrashekar2014survey}.
However, it should be noted that existing supervised FS methods are facing an enormous challenge --- the generation of reliable supervised knowledge cannot catch up with the rapid growth of newly-emerging concepts and multimedia data.
%In other words, as illustrated in Fig.~\ref{fig_problem}, it is difficult to collect labeled instances for all the existing and coming categories XXXX.
In practice, it is costly to annotate sufficient training data for new concepts timely, and meanwhile, impractical to retrain the FS model whenever a new concept emerges.
%whereas the retrieval system meets a new concept. wasteful/expensive/uneconomical
As illustrated in Fig.~\ref{fig_problem}, traditional methods perform well on the seen concepts which have correct guidance, but they may easily fail on the unseen concepts which have never been observed, like the newly invented product ``quadrotor''.
% they nev-er meet before such as the “dicycle” which is a kind of vehicle
%In other words, as illustrated in Fig.~\ref{fig_problem}, due to the rapid growth of newly-emerging concepts and multimedia data, it is impossible to obtain labeled samples for all classes, such as the new invented product ``quadrotor''.
%rapid increasing speed of newly-emerging semantic concepts and multimedia data.
%We call this problem as Zero-Shot Feature Selection Problem.
%We address the feature selection task in zero-shot setting: the test data are coming from unseen classes.
% problem of zero-shot event recognition in consumer videos.
%This challenge motivates us to consider: whether we can design a feature selection strategy to handle the multimedia data coming from unseen categories.
%This challenge motivates us to consider: whether we can design a feature selection strategy to handle the coming unseen categories.
%The key is to transfer the supervised knowledge from the ``seen'' categories to the ``unseen'' categories.
%However, xxxxxxx .
Therefore, the problem of \emph{Zero-Shot Feature Selection (ZSFS)}, i.e., building a FS model that generalizes well to unseen concepts with limited training data of seen concepts, deserves great attention.
%is very important for real-world applications.
%building generalizable feature selection model that can handle unseen concepts
%, i.e., identifying key features for the coming unseen concepts with limited training data of seen concepts, is very important for real-world applications.
%Therefore, building generalizable feature selection model which can identify the key features for unseen concepts is very important for real-world applications.
%However, existing works pay little attention to this problem.
However, few studies have considered this problem.
%However, little attention has been paid to this problem.

\begin{figure}[!t]
\centering
    \includegraphics[width=0.39\textwidth]{images/problem.pdf}
\caption{
%Illustration of Zero-Shot Feature Selection Problem.}
%An example of newly-emerging concepts to the existing learning systems.
%The Zero-Shot Feature Selection Problem. The feature selection model trained with seen concepts should generalize well to unseen concepts.
%Illustration of the Zero-Shot Feature Selection Problem.
The Zero-Shot Feature Selection Problem.
%, i.e., building the feature selection model that generalizes well to unseen concepts with limited training data of seen concepts.
}
\label{fig_problem}
\end{figure}

%In this paper, we formally study this \emph{Zero-Shot Feature Selection (ZSFS)} problem which aims to build feature selection model which can handle the xxx of unseen concepts.
%capture the similarity structure of both seen and unseen concepts.
The major challenge in the ZSFS problem is how to deduce the knowledge of unseen concepts from seen concepts.
In fact, the primary reason why existing studies fail to handle unseen concepts is that they only consider the discrimination among seen concepts (like the 0/1-form class labels illustrated in Fig.~\ref{fig_problem}), such that little knowledge could be deduced for unseen concepts.
%reflected/depicted
%(like the 0/1-form class labels in Fig.~\ref{fig_problem})
%all prefer the features best reflecting the discrimination (like the 0/1-form label vectors in Fig.~\ref{fig_problem}) among seen concepts.
%As such, little knowledge about unseen concepts is deduced.
%they treat all concepts independently, like the 0/1-form label vectors shown in Fig.~\ref{fig_problem}.
%As such, labels only reflect the discrimination among seen concepts but provide little information about unseen concepts.
%In this way, the label vectors only reflect the discrimination among seen concepts, and provide little in
%In this way, each concept cannot leverage the knowledge from other related concepts or contribute its own knowledge to others.
%only reflect its own information, and cannot provide any knowledge to the others.
%cannot leverage the knowledge from other related concepts or contribute its own information to the others.
%To alleviate this, in this paper, we propose to utilize the semantic descriptions xxxx to ....
%%, and propose a novel method, termed \emph{Semantic based Zero-Shot Feature Selection (\myalg)}.
To address this, as illustrated in Fig.~\ref{fig_method}, we adopt the class-semantic descriptions (i.e., attributes) as supervision for FS model learning.
%we adopt the class-semantic descriptions (i.e., attributes) as side information for the ZSFS problem.
%semantic vectors of concepts
%class-attribute descriptors
%we propose to replace the original 0/1-form class labels with attribute descriptions, i.e., the knowledge about some attributes of seen concepts (e.g., ``has stripes'', ``can fly'' and ``is metal'').
%This idea is inspired by the recent development of Zero-Shot Learning (ZSL)~\cite{farhadi2009describing,akata2016multi} which has demonstrated that by leveraging an intermediate semantic description shared between seen and unseen categories, i.e., attributes, supervised knowledge can be transferred from the seen concepts to unseen concepts.
%This idea is inspired by the recent development of Zero-Shot Learning (ZSL)~\cite{farhadi2009describing,akata2016multi}.
This idea is inspired by the recent development of Zero-Shot Learning (ZSL)~\cite{farhadi2009describing,akata2016multi} which has demonstrated that the capacity of inferring attributes allows us to describe, compare, or even categorize unseen objects.
%More concretely, recent ZSL studies have demonstrated that the capacity of inferring attributes allows us to describe, compare, or even categorize unseen objects.
%More concretely, recent ZSL studies have demonstrated that by leveraging an intermediate attribute layer shared between seen and unseen concepts, supervised knowledge can be transferred from the seen concepts to unseen concepts.
%As such, we expect the selected features to have the discriminative power of categorizing unseen objects via learning the relationship between features and attributes.
%As such, we expect the selected features to have the discriminative power to categorize unseen objects by learning the relationship between features and attributes.

An attendant problem is how to identify reliable discriminative features with attributes which might be inaccurate and noisy~\cite{jayaraman2014zero}.
To alleviate this, we further propose a novel loss function (named \emph{center-characteristic loss}) which encourages the selected features to capture the central characteristics of seen concepts.
%Theoretically, this loss function can be seen as a variant of the center loss regularization~\cite{wen2016discriminative} which has shown its effectiveness for learning discriminative and generalized features, so as to categorize unseen objects.
Theoretically, this loss function is a variant of the \emph{center loss}~\cite{wen2016discriminative} which has shown its effectiveness to learn discriminative and generalized features for categorizing unseen objects.


%we modify the regularized center loss~\cite{wen2016discriminative} which has shown minimize the distances
%between the learned features and their corresponding class
%centers
%we further propose a novel loss function (named \emph{center-characteristic loss}) which encourages the selected features to capture the central characteristics of seen concepts.
%%In addition, to identify more reliable discriminative features, we further propose a novel loss function (named \emph{center-characteristic loss}) which encourages the selected features to capture the central characteristics of seen concepts.
%%whose goal is to select the features lying the center of seen classes.
%%Finally, we formulate these
%%Finally, we formulate these two components into a unified optimization framework and present an efficient solution.
%Finally, we combine these two components into a joint learning model, and present an efficient optimization method.


%In this paper, we propose a novel ZSFS method, termed as \emph{Semantic based Feature Selection (\myalg)}.
%%As demonstrated in the success of Zero-Shot Learning (ZSL)~\cite{lampert2009learning}~\cite{farhadi2009describing},
%Our method is inspired by the recent development of Zero-Shot Learning (ZSL)~\cite{lampert2009learning,farhadi2009describing} which has demonstrated that by leveraging an intermediate semantic description shared between seen and unseen categories, i.e., attributes, supervised knowledge can be transferred from the seen concepts to unseen concepts.
%Specifically, as illustrated in Fig.~\ref{fig_method}, we propose to replace the original 0/1-form class labels with semantic attribute labels, i.e., the knowledge about some attributes of seen concepts (e.g., ``has stripes'', ``can fly'' and ``is metal'').
%%As attributes connect the seen and unseen classes, the knowledge of unseen classes is introduced in this way.
%%As attributes bridge the seen and unseen classes, supervised knowledge would be successfully transferred from the seen classes to unseen classes.
%%We expect to identify the features which capture the discrimination of attributes ,
%As such, we expect the selected features to have the discriminative power of categorizing unseen objects via learning the relationship between features and attributes.
%%As illustrated in Fig.~\ref{fig_example}, to transfer the knowledge to the coming unseen classes for feature selection, we propose to replace the original class labels with semantic attribute labels, i.e., the knowledge about some attributes of seen classes (e.g., ``has stripes'', ``can fly'' and ``is metal'').
%%The key is how to set up a bridge to transfer supervised knowledge between ``seen'' and ``unseen'' categories.
%%
%%Recent development of Zero-Shot Learning (ZSL)~\cite{lampert2009learning}~\cite{farhadi2009describing} demonstrates that by leveraging an intermediate
%%semantic description shared between seen and unseen categories, i.e., attributes, supervised knowledge can be transferred from the seen classes to unseen classes.
%%%they are also capable of detecting completely unseen classes when provided with a high-level description.
%%Inspired by this idea, in this paper, we propose a novel feature selection method, termed \emph{Semantic based Zero-Shot Feature Selection (\myalg)}.
%%As illustrated in Fig.~\ref{fig_example}, to transfer the knowledge to the coming unseen classes for feature selection, we propose to replace the original class labels with semantic attribute labels, i.e., the knowledge about some attributes of seen classes (e.g., ``has stripes'', ``can fly'' and ``is metal'').
%%of unseen classes is introduced in this way.
%%Since these attributes provide discriminative semantic properties of unseen classes, the selected features should also have this discriminative power.
%%we propose to replace the original
%%project the original supervised knowledge from the independent label space into semantic attribute space.
%%to bridges gaps between seen and unseen classes, we project the original supervised knowledge from the independent label space into semantic space.
%%Afterwards, the features, which can distinguish these attributes, are selected for the coming unseen classes.
%%Since these attributes provide discriminative semantic properties of unseen classes, the selected features should also have this discriminative power.
%%they can be used in the training phase to select useful features for the images of unseen classes.
%%they can be used to select useful features for the images of unseen classes.
%%we select the features which could best generate these semantic representations.
%%In other words, the features, which can distinguish various attributes of seen classes, are selected for the coming unseen classes.
%%In other words, we select features that can distinguish different attributes which has the capability to describe unseen categories.
%%Since these semantic represents are corrlated/shared in the classes of both seen and unseen categories, these selected features could capture xxxx.
%In addition, to identify more reliable discriminative features, we further propose a novel loss function (named \emph{center-characteristic loss}) which encourages the selected features to capture the central characteristics of seen concepts.
%%whose goal is to select the features lying the center of seen classes.
%%Finally, we formulate these
%%Finally, we formulate these two components into a unified optimization framework and present an efficient solution.
%Finally, we combine these two components into a joint learning model, and present an efficient optimization method.

%We evaluate the performance of the proposed method on several real-world datasets, including SUN, aPY and CIFAR10.
%One point should be noted is that the attributes of CIFAR10 are automatically generated from a public Wikipedia text-corpus~\cite{shaoul2010westbury} by a well-known NLP tool~\cite{huang2012improving}.
%%The experimental results show that
%The experimental evidence shows that no matter with manually or automatically generated attributes, our method generalizes well to unseen concepts.
%our method could build a generalizable feature selection model that can identify key features for unseen concepts.
%In practical usage, most supervised feature selection methods~\cite{nie2010efficient}~\cite{cai2013exact} require training examples of all testing classes, i.e., all testing images should belong to the ``seen'' classes.
%%However, traditional super-vised methods have been facing an enormous challenge, i.e., the generation of reliable supervised knowledge cannot catch up with the rapid increasing speed of newly-emerging semantic concepts and multimedia data.
%%~\cite{lee1988thirteen}
%%However, little work has considered a more challenging case where testing data belongs to some related but ``unseen'' classes.
%However, little work has considered a more challenging problem where testing data comes from some ``unseen'' classes, i.e., the \textbf{Zero-Shot Feature Selection Problem} (illustrated in Fig.~\ref{fig_problem}).
%%However, few work considers a more practical and challenging case where testing images come from the ``unseen'' categories.
%%Actually, this case has practical importance.
%This problem deserves special attention for two reasons.
%%, due to the rapid growth of newly-emerging concepts and multimedia data.
%%On one hand, within the ``seen'' area where images are attached with known classes, existing supervised feature selection algorithms may perform well with correct guidance.
%%On the other hand, we also wish the learned knowledge could generalize to data of new classes which are never observed, such as uncommon animals and new invented products.
%%As illustrated in Fig.~\ref{fig_example},
%On the one hand, existing supervised feature selection algorithms, which learn from the seen classes, may easily fail to generalize to the data of new
%classes that have never been observed.
%On the other hand, due to the rapid growth of newly-emerging concepts and multimedia data, it is impossible to obtain labeled samples for all classes, such as the uncommon animal ``koala'' and new invented product ``quadrotor''.
%%As illustrated in Fig.~\ref{fig_example}, within the ``seen'' part where images are attached with known classes, existing supervised feature selection algorithms may perform well with correct guidance.
%%On the other hand, due to the rapid growth of newly-emerging concepts and multimedia data, it is impossible to obtaining labeled examples for all classes, such as the uncommon animal ``koala'' and new invented ``quadrotor''.
%%we also wish the learned knowledge could generalize to data of new classes which are never observed, such as the uncommon animal ``koala'' and new invented ``quadrotor''.
%%Nevertheless, outside the seen area, the learned knowledge may fail to generalize to data of new classes that they never observe.
%%One typical application is image feature selection, where tens of thousands of objects which we might want to analysis.
%%One obvious example is image processing, where there are tens of thousands of objects which we might want analysis.
%%This motivates us to consider how to utilize the limited training images of seen categories to design feature selection towards unseen categories.
%%Therefore, we must have a way to design a feature selection strategy for the multimedia data beyond those in the training set.
%%This motivates us to consider whether we can utilize the existing labeled samples of seen categories to guide the feature selection for the coming unseen categories.
%%This motivates us to consider how to design the feature selection method for the coming unseen categories.
%%Therefore, we may wonder: how to handle the coming unseen categories, using limited training samples of seen categories.
%%This motivates us to consider: how to design the feature selection strategy to deal with the coming unseen categories (or at least in some specific application scenarios).
%This motivates us to consider: in practical applications, could we design a feature selection strategy to handle the coming unseen categories?
%
%
% utilize the limited training samples of seen categories to  deal with unseen objects.


%The key challenge is how to transfer supervised knowledge from ``seen'' classes to ``unseen'' classes.

%, because of the expensive cost of manually labeling and the rapid
%However, due to the expensive cost of manually labeling and the explosion of xxxx, it is impossible to generate label examples for every newly-emerging semantic concepts and multimedia data.
%For example, when unseen objects, such as uncommon animals or medical scans, are confronted.
%Existing work fails to handle this problem.
%
%where images are attached with known categories, existing super-vised hashing algorithms may perform well because they are fed
%with correct guidance.



%\begin{figure}[!t]
%\centering
%    \includegraphics[width=0.5\textwidth]{images/www}
%\caption{Illustration of Zero-Shot Feature Selection.}
%\label{fig_example2}
%\end{figure}

%Actually, this case has many practical applications.
%For example, we plan to perform feature selection in some uncommon categories, such
%as “otter” and “koala”, which are hard to obtain labeled
%samples. On the other hand, collecting labeled training data
%in some common categories, like “cat” and “dog”, is much
%easy.
%cost of obtaining labeled examples for all values is high.
%One obvious example is computer vision, where there are tens of thousands of objects which we might want analysis.
%we must have a way to extrapolate to recognizing words beyond those in the training set.
%This motivates us to consider whether we can utilize the existing labeled samples of seen categories to guide the feature selection for the newly-emerging unseen concepts and multimedia data


\begin{figure}[!t]
\centering
    \includegraphics[width=0.47\textwidth]{images/example_new.pdf}
%\caption{Overview of the proposed method for the ZSFS problem.}
\caption{Overview of the proposed method.}
\label{fig_method}
\end{figure}


%with one unified formulation
%Finally, we formulate these two claims into a unified optimization problem and present an efficient solution.
%introduces pseudo labels to the target domain via knowledge transferring from source domain
%%Figure~\ref{fig_example} illustrates the .
%Specifically, our method not only introduces pseudo labels to the target domain via knowledge transferring from source domain, but also ensures these labels preserve the manifold structure of the target data.
%Besides, we jointly consider the information from source domain and target domain to archive better performance.
%In summary, we make the following contributions in this paper:
We summarize our main contributions as follows:
%Our main contributions are summarized as follows:
\begin{itemize}\setlength{\itemsep}{-0.0cm}
  \item
  %We study the problem of employing training data of seen categories to select discriminative features for unseen categories.
  %We study the problem of selecting features for unseen categories with limited training data of seen categories.
  %We study the problem of feature selection towards the images of unseen classes with limited training data of seen classes.
  We study the problem of ZSFS.
  %, i.e., building a feature selection model which generalizes well to unseen concepts with limited training data of seen concepts.
  %, i.e., identifying key features for the coming unseen concepts with limited training data of seen concepts.
  To our best knowledge, little work has addressed this problem.
  %this is the first attempt to study the problem of selecting features for the unseen categories with limited seen supervised knowledge.
  \item We propose an efficient strategy to reuse the supervised knowledge of seen concepts.
    Concretely, feature selection is guided by the seen concept attributes which provide discriminative information about unseen concepts.
%  Concretely, we use semantic attribute labels of seen classes to guide feature selection.
%  Since these attributes provide discriminative information about unseen classes, the selected features should also has this discriminative power.
%  we project the original binary label vectors of seen data to semantic attribute space where unseen categories can be distinguished by these attributes.
%  %Then, the features which could best generate these semantic representations are selected for the coming unseen classes.
%  %, and select the features best xxx semantic meaning.
%  Guided by these semantic knowledge, selected features have discriminant power to distinguish unseen classes.
  %in which semantic correlations among labels unseen categories xxxxx.
%  transfer the supervised knowledge from seen categories to unseen categories.
%   Specifically, we projecting the original label information to semantic embedding space, in which the unseen categories xxxxx.
  \item To select more reliable discriminative features, we propose a new loss function (called center-characteristic loss) to encourage the selected features to capture the central characteristics of seen concepts.
%  To select more reliable discriminative features, we further encourage the selected features to capture the central characteristics of seen concepts.
%  %We further formulate this purpose by a novel loss function named center-characteristic loss.
%  %We formulate this by a novel loss function named center-characteristic loss.
%  This is formulated as the center-characteristic loss.
%  This intuition is captured by a new proposed loss function named center-characteristic loss.
%  propose another new loss function (called center-characteristic Loss).
%  This is the first attempt to use such a loss function enhance the generalizing power of selected features for the coming unseen classes.
  %To be best of our knowledge, this is the first attempt to use such a loss function to select discriminative features for unseen categories.
  \item
%  In order to generate more reliable discriminative features, we propose a new loss function (called self-center loss) to minimize the intra-class distances of the deep features.
  We conduct extensive experiments on three benchmark datasets to demonstrate the effectiveness of our method.
  %the proposed method.
  %We conduct extensive experiments on three benchmark datasets. The experimental results indicate that our algorithm consistently outperforms other compared algorithms on all the databases.
\end{itemize}


%The rest of this paper is organized as follows. In Section 2, we briefly review some related work on feature selection and zero-shot learning.
%In Section 3, we will elaborate our approach with details, together with our optimization method and an analysis of the method.
%Extensive experiments on several different datasets will be reported in Section 4, followed by the conclusion in Section 5.



==> others_new.tex <==
\subsection{Orthogonality variance add}
\begin{equation}
\label{eq_final_cost}
\begin{aligned}
\underset{W, \sigma}{\text{min\ }} & \mathcal{J} = \left \| (Y_{s}{-}XW) \rm{diag}(\sigma) \right \|^{2}_{F} + \gamma \left \| W \right \|_{21} + \lambda \left \| \sigma \right \|^{2}_{F} \\
\mathrm{s.t.}   & \hspace{0.5em} \sigma \ge 0,\ \sigma^{T}1_{d}=1
\end{aligned}
\end{equation}
where $\sigma \in R^{d \times 1}$, $\sigma >= 0$ and $\sum \sigma = 1$ to avoid trivial solution is the variance vector.
We can denote $\Sigma = diag(\sigma)$.

\subsubsection*{Fix $W$, and update $\sigma$}
We define $A = Y_{s}{-}XW$, remove the irrelevant functions, and get:
\begin{equation}
\label{eq_final_cost}
\begin{aligned}
\underset{\sigma}{\text{min\ }} & \mathcal{J} = \left \| A \rm{diag}(\sigma) \right \|^{2}_{F} + \lambda \left \| \sigma \right \|^{2}_{F} \\
\mathrm{s.t.}   & \hspace{0.5em} \sigma \ge 0,\ \sigma^{T}1_{d}=1
\end{aligned}
\end{equation}


\begin{equation}
\label{eq_derive_W}
\begin{aligned}
& \mathcal{J}_{\sigma} = \sum_{i=1}^{a}\sigma^{2}_{i} { \sum_{k=1}^{n}A^{2}_{ik} } + \lambda \left \| \sigma \right \|^{2}_{F} \\
&\frac{\partial \mathcal{J}}{\partial W} = -2(X\mathrm{diag}(s))'Y_{s} + 2(X\mathrm{diag}(s))'(X\mathrm{diag}(s))W\\
\end{aligned}
\end{equation}

==> our_method_L1_center_ijcai.tex <==

\input{preliminary_problem}

\section{The Proposed Method}\label{sect_method}
%%In this section, we provide the detail
%%In this section, we provide a complete description of the proposed method \myalg.
%In this section, we provide a detailed description of the proposed method \myalg.
%%In this section, we provide details about the proposed \myalg\ method.
%Firstly, we discuss the feasibility of transferring knowledge to unseen concepts from seen concepts.
%Then, we describe the formulation of \myalg\ method.
%Finally, we provide an effective solution to address the optimization issue of \myalg.
%%Finally, we analyse the computational complexity of the optimization method.

%In this section, we provide a detailed description of the proposed method.
%Firstly, we discuss the feasibility of transferring knowledge to unseen concepts from seen concepts.
%Then, we describe the formulation of our method.
%Finally, we provide an effective solution to address the involved optimization issue.
%In this section, we present the proposed ranking based
%factorization method for POI recommendation. We first
%formulate the POI recommendation problem by a ranking
%objective function, and then introduce how to optimize it.
%Finally, we generalize the model for time-aware POI recommendation.

\subsection{Deduce Knowledge for Unseen Concepts}
%As mentioned above, the key idea is to reuse the supervised knowledge of seen classes for the coming unseen classes.
%On the other hand, class labels usually have semantic meanings, like ``cat'' and ``dog''.
%According to theory of ZSL, seen class labels can be described via semantic descriptions xxxx.
%In other words, ZSL approaches take attributes as an intermediate bridge to transfer knowledge from seen classes to unseen classes.
%At the testing stage, after successfully inferring the attributes of the unseen images, we can classify unseen classes such as ``koala'' and ``helicopter'' without any training images.
%With this learned knowledge, we can infer the attributes of unseen class ``koala'' and ``helicopter'', so as to classify them without any training images.
The success of ZSL demonstrates that the capacity of inferring attributes allows us to describe, compare, or even categorize unseen objects.
%In light of this, we use attribute representation to replace with the original independent binary label information.
%In light of this, as illustrated in Fig.~\ref{fig_example}, we project the original binary labels to semantic representation space.
In light of this, as illustrated in Fig.~\ref{fig_method}, we propose to use class-attribute descriptions to guide feature selection.
%replace the original class labels with class-attribute descriptions to guide feature selection.
In other words, we prefer the features which are important for recognizing the attributes of seen concepts.
%have the ability of recognizing the attributes of seen concepts.
%are useful for recognizing the attributes of seen concepts.
%(short for \emph{attributes})
%we use attribute labels to replace the original labels, so as to further guide feature selection.
%Compared to the original class labels, attributes not only reflect the differences among seen concepts but also provide additional semantic information about unseen concepts.
Unlike the original class labels (e.g., the 0/1-form label vectors in Fig.~\ref{fig_problem}) which only reflect the discrimination among seen concepts, attributes provide additional semantic information about unseen concepts, making the FS models trained with seen concepts generalize well for unseen concepts.
%In this way, the supervised knowledge from one concept can contribute to other concepts.
%Consequently, the FS model trained with the attribute descriptions of seen concepts could generalize well to unseen concepts.
%
% the supervised knowledge
%
%selected features would capture the discriminative power of categorizing unseen objects via attributes.
%
%by introducing attributes, .
%Therefore, by introducing attributes, we hope to transfer the supervised knowledge from the seen concepts to unseen concepts..
%
%can transfer the supervised knowledge from the seen concepts to unseen concepts.
%% discriminative information
%%In this way, supervised knowledge are successfully transferred from the seen classes to unseen classes.
%In other words, by introducing attributes, we can transfer the supervised knowledge from the seen concepts to unseen concepts.
%For example,
% by these attribute labels.
%After that, feature selection is guided by these attributes.
%Since these attributes provide discriminative semantic descriptions about the unseen categories, the selected features should also have this discriminative power.
%use attribute representation to replace with the original independent binary label information.
%Specifically, for each seen class type, we replace the original binary labels with its attribute representation vector.
%In this semantic space, semantic correlations among different classes can be quantitatively measured and captured.
%These attributes provide semantic information about the unseen categories.
%Every class label is described by pure text.
%In the subsequent part, we denote the used semantic attribute labels as $Y_{s} {\in} \mathbb{R}^{n, a}$, where $a$ is the attribute number.


%In this paper, we use xxx to denote the attribute description vectors of seen concepts $\mathcal{C}^{s}$.
Suppose the attribute descriptions of all seen concepts in $\mathcal{C}^{s}$ are given.
For brevity, we denote the corresponding semantic label knowledge of seen instances (i.e., $X$) as $Y_{s} = [y^{s}_{1}, ..., y^{s}_{n}]' \in \mathbb{R}^{n \times m}$, where $y^{s}_{i} \in \mathbb{R}^{m}$ denotes the attribute description of the seen concept which instance $x_{i}$ belongs to, and $m$ is the attribute number.
%for each seen concept $c \in \mathcal{C}^{s}$, we use
%we assume the class-attribute description
%In the subsequent part, we denote this kind of semantic knowledge as $Y_{s} {\in} \mathbb{R}^{n \times m}$, where $m$ is the attribute number.
%In the subsequent part, we denote the used attribute labels as $Y_{s} {\in} \mathbb{R}^{n \times m}$, where $m$ is the attribute number.
%These attributes can either be provided manually or generated automatically from online textual documents~\cite{rohrbach2010helps}, such as Wikipedia articles.
%In other words, each seen class is described by a xxxxxx.~\cite{qiao2016less}
%With these Then we can select features best
%After that, if we can select the features which best distinguish these attributes.
%Since these attributes provide semantic information about the unseen categories, with these attributes, the selected features should also have this generalizing power.
%Since these attributes have the capability to distinguish the coming unseen classes, the selected features should also have this generalizing power.
%When an unseen object shows up, these attribute discriminative features are capable to categorize unseen objects in a semantic level.
%When learning the attributes, we could generalize to new types of objects
%the seen class labels can be projected into the semantic space.
%This is because attributes are shared across different categories and provide a compact but discriminative representation.
%Therefore, unseen labels can
%leverage the well-established mapping from its semantically close
%seen categories.
%In this paper, we adopt pure textual descriptions as attributes to describe seen class labels.
%These attributes can either be manually given or .

\subsection{Zero-Shot Feature Selection}
\paragraph{Feature selection with attributes}
%With the used semantic labels, the feature selection procedure is described as follows.
%we can perform feature selection.
%Recall that we intend to use the amendatory supervised knowledge to guide the feature selection $Y_{s}$.
We use $s {=} \{0, 1\}^{d}$ as the indicator vector, where $s_{i} $=$ 1$ if the $i$-th feature is selected and $s_{i} $=$ 0$ otherwise.
%Let us denote the diagonal matrix with diagonal elements $s$ as $diag(s)$.
%Diag(s) denotes the matrix with the main diagonal beings
Denoting $\mathrm{diag}(s)$ as the matrix with the main diagonal being $s$, the original data can be represented as $X\mathrm{diag}(s)$ with the selected features.
%Then, the original data can be represented as $X\mathrm{diag}(s)$ with the selected features.
%Therefore, the new representation of training example constructed by the selected features is $X\mathrm{diag}(s)$.
%Therefore, the selected features comprise a new representation of training example, and we denote it as $X\mathrm{diag}(s)$.
% can be represented as $ X' = X\mathrm{diag}(s)$.
From a generative point of view, we assume that the selected features should have the ability to generate the given attributes.
%We further assume that these selected features could generate the amendatory supervised knowledge $Y_{s}$.
For simplicity and efficiency, we use a linear generating function $W {\in} \mathbb{R}^{d \times m}$, and adopt the squared loss to measure the error.
%Then the generation can be captured by the following optimization problem:
%Therefore, the optimal $s$ is given by the following optimization problem:
Therefore, the optimal $s$ can be obtained by solving the following minimization problem:
%Thus, the feature selection problem can be captured by the following optimization problem:
%Recall that we intend to use the amendatory supervised knowledge to guide the feature selection $Y_{s}$, the generation can be captured by the following optimization problem:
%\begin{equation}
%\label{eq_basic_source}
%\begin{aligned}
%\underset{f}{\text{min }} & \sum_{i=1}^{n_{s}}\mathcal{L}(f(x_{i}\mathrm{diag}(s)),y_{si}) + \mathcal{R}(f) \\
%\mathrm{s.t.}   & \hspace{0.5em} s \in \{0,1\},\ s^{T}\textbf{1}_{d}=k
%\end{aligned}
%\end{equation}
%where $\mathcal{L}(\cdot,\cdot)$ is a loss function, $f$ is the learned classifier, and $\mathcal{R}$ is the regularization term for $f$ to avoid overfitting.

\begin{equation}
\small
\label{eq_semantic_selection}
\begin{aligned}
\underset{W, s}{\text{min }} & \mathcal{J}_{1} = \left \| Y_{s}-X\mathrm{diag}(s)W \right \|^{2}_{F} + \gamma \left \| W \right \|^{2}_{F} \\
\mathrm{s.t.}   & \hspace{0.5em} s \in \{0,1\}^{d},\ s^{T}\textbf{1}_{d}=k
\end{aligned}
\end{equation}
where $k$ is the number of selected features, $\gamma$ is the regularization parameter to avoid overfitting, and $\textbf{1}_{d}$ is a column vector with all its elements being 1.
The most important part of Eq.~\ref{eq_semantic_selection} is the attributes $Y_{s}$ through which the power of categorizing unseen objects is captured by the selected features.
%which would make the selected features to have the discriminative power of categorizing unseen objects.
%The benefit of the above formulation is that it can narrow down the semantic gap between seen and unseen classes.
%The benefit of the above approach is that the selected features would capture the discriminative power of categorizing unseen objects via attributes.

%Problem~\ref{eq_semantic_selection} can be seen as the classical ($\ell_{1}$-norm based) Lasso problem with the modified supervised knowledge.
%By finding the solution that minimize Eq.~\ref{eq_semantic_selection}, we select $k$ features which best generate semantic labels (descriptions) of seen classes.
%select features that are beneficial in learning attribute classifiers.
%We can even learn new categories withnovisual examples, using textual de-scriptions instead.

\paragraph{The center-characteristic loss}
%\begin{figure}[htbp]
%\centering
%    \includegraphics[width=0.4\textwidth]{images/center_loss.pdf}
%\caption{Separable Features vs. Discriminative Features (center loss) \protect\cite{wen2016discriminative}.}
%\label{fig_center-loss}
%\end{figure}

\begin{figure}[!t]
\centering
    \includegraphics[width=0.47\textwidth]{images/center_character_loss_IJCAI.pdf}
%\caption{Center loss \protect\cite{wen2016discriminative} vs. center-characteristic loss.}
\caption{Center loss vs. Center-characteristic loss.}
\label{fig_center-loss}
\end{figure}

Although introducing attributes seems to be an effective solution for the ZSFS problem, it still has some limitations for discriminative feature selection.
%Although attributes seem a very efficient solution for the ZSFS problem, attributes still has some limitations.
%have the capability of categorizing unseen classes, attributes still has some limitations.
Firstly, attributes cannot naturally describe the uncertainty about a class whose appearance may vary significantly~\cite{ren2016joint}.
%whose instances usually appear differently~\cite{ren2016joint}.
%which is visually distinguished
%which may show different .
%This is because that even though various images belong to the same class, uncertainty is associated with them.
For instance, ``televisions'' may have different colors and look quite differently from different angles.
% through different perspectives
%have quite different appearances through different perspectives.
Moreover, attributes, which can be seen as real-valued multi-labels, tend to be more noisy compared to the common single-class labels~\cite{jayaraman2014zero}.
% contain more noise compared to the binary single-labeled data. binary single-labels
For example, it is hard to determine a proper score for the attribute ``running fast'' for different animals and man-made vehicles.
%These limitations would negatively affect the discrimination of selected features.
%These limitations would negatively impact the discrimination feature selection.
% the quality of the selected features.
%These limitations would confuse the feature selection model to identify discriminative features.

Recent work of supervised feature learning~\cite{wen2016discriminative} has pointed out that discriminative features are more generalized for identifying unseen objects than separable features.
%Specifically, as illustrated in Fig.~\ref{fig_center-loss}, center loss minimizes the distances between the learned features and their corresponding class centers.
Specifically, to learn discriminative features, \cite{wen2016discriminative} introduces \emph{center loss} to minimize the distances between the learned features and their corresponding class centers (as illustrated in the upper portion of Fig.~\ref{fig_center-loss}).
%has pointed out that the learned features should close to their corresponding class centers
%The learned features need to be not only separable but also discriminative...
%generalized enough for identifying new unseen
%As illustrated in Fig.~\ref{fig_center-loss}, discriminative features better compact intra-class variations and distinguish inter-class differences.
%As shown in Fig.~\ref{fig_center-loss}, discriminative features better compact intra-class variations and distinguish inter-class differences.
%Motivated by this, we force the the selected features should be close to their corresponding class centers.
%Accordingly, we minimize the distances between the selected features and their corresponding class centers, which yields the following minimization problem:
Accordingly, for the FS task, this loss minimizes the distances between the selected features and their corresponding class centers, which yields the following minimization problem:
%by minimizing the following objective function.
%encourage to select the features lying close to their corresponding class centers.
%This minimizes the following objective function:
%we introduce a new loss function for feature selection, \emph{self-centeredness loss}, namely the selected features should be close to their corresponding class centers.
\begin{equation}
\small
\label{eq_center-loss}
\begin{aligned}
\underset{s}{\text{min }} & \mathcal{J}_{2} = \left \| X\mathrm{diag}(s) -\bar{X}\mathrm{diag}(s) \right \|^{2}_{F} \\
%\sum_{i=1}^{n}\left \| x_{i}\mathrm{diag}(s) -\bar{x}_{i}\mathrm{diag}(s) \right \|^{2}_{F} \\
\mathrm{s.t.}   & \hspace{0.5em} s \in \{0,1\}^{d},\ s^{T}\textbf{1}_{d}=k
\end{aligned}
\end{equation}
%where $\bar{x}_{i}$ is the denotes the $y_{i}$-th class center of features.
%where $\bar{X} = \{\bar{x}_{1}, ..., \bar{x}_{n} \}'\in \mathbb{R}^{n \times d}$, and $\bar{x}_{i}$ denotes the feature vector of the $y_{i}$-th class center.
where $\bar{X} = \{\bar{x}_{1}, ..., \bar{x}_{n} \}'\in \mathbb{R}^{n \times d}$, and $\bar{x}_{i}$ denotes the feature vector center of the class which $x_{i}$ belongs to.
%$\bar{x}_{i}$ denotes the $y_{i}$-th class center of features.

However, this constraint may be too strict for a FS task, since all features are pre-calculated.
%extracted.
On the other hand, as our ultimate goal is to find the relevance between features and attributes, it is reasonable to incorporate the attributes into this loss function.
% we need to move towards generating more integrative models
Therefore, we modify this constraint by multiplying the terms in the square loss with the generating function $W$ and approximate $X\mathrm{diag}(s)W$ with $Y_{s}$ according to Eq.~\ref{eq_semantic_selection}.
%This modification make xxxx connection xxxx, which xxxxx.
%, as XXXXXXXXXX for some reasons
%Finally, we get the following loss function:
%After this modification, Eq.~\ref{eq_center-loss} becomes:
After these modifications, Eq.~\ref{eq_center-loss} becomes:
\begin{equation}
\small
\label{eq_self-center-loss}
\begin{aligned}
\underset{W,s}{\text{min }} & \mathcal{J}_{2} = \left \| Y_{s}-\bar{X}\mathrm{diag}(s)W \right \|^{2}_{F}  \\
\mathrm{s.t.}   & \hspace{0.5em} s \in \{0,1\}^{d},\ s^{T}\textbf{1}_{d}=k
\end{aligned}
\end{equation}

We call this loss function \emph{center-characteristic loss}, as it encourages the selected features to capture the central characteristics of seen concepts (illustrated in the lower portion of Fig.~\ref{fig_center-loss}).
%Meanwhile, xxxx to attributes.
%Intuitively, this xxxx aims to.
%compacts intra-class variations
%it encourages the selected features to lie in
% encourages diversity between individual predictors of an ensemble
%compact intra-class variations
%namely for each class, the selected feature should close to the class center.
%%Intuitively, this loss function ensures the selected features should lie in the cluster centers.
%Intuitively, the features which capture the central characteristics of seen classes are preferred.


%namely the selected features should not only separable but also discriminative.
%In other words, the selected feature should tend to self-centeredness.
%Feature center loss should show lower intra-class variations.

\paragraph{Zero-Shot feature selection joint learning model}
%\subsubsection{The Unified Model: \myalg}
By combining the objective functions in Eqs.~\ref{eq_semantic_selection} and~\ref{eq_self-center-loss}, the proposed method is to solve the following optimization problem:
%\textbf{Final:}
%\begin{equation}
%\small
%\label{eq_final_cost01}
%\begin{aligned}
%\underset{W, s}{\text{min }} & \mathcal{J} {=} \left \| Y_{s}{-}X\mathrm{diag}(s)W \right \|^{2}_{F} {+} \alpha \left \| Y_{s}{-}\bar{X}\mathrm{diag}(s)W \right \|^{2}_{F} {+} \gamma \left \| W \right \|^{2}_{F} \\
%\mathrm{s.t.}   & \hspace{0.5em} s \in \{0,1\}^{d},\ s^{T}\textbf{1}_{d}=k
%\end{aligned}
%\end{equation}
\begin{equation}
\small
\label{eq_final_cost01}
\begin{aligned}
\underset{W, s}{\text{min }} & \mathcal{J} = \left \| Y_{s}{-}X\mathrm{diag}(s)W \right \|^{2}_{F} {+} \alpha \left \| Y_{s}{-}\bar{X}\mathrm{diag}(s)W \right \|^{2}_{F} \\
& \hspace{2em} + \gamma \left \| W \right \|^{2}_{F} \\
\mathrm{s.t.}   & \hspace{0.5em} s \in \{0,1\}^{d},\ s^{T}\textbf{1}_{d}=k
\end{aligned}
\end{equation}
where $\alpha$ is a balancing parameter. We call the proposed method as \emph{Semantic based Feature Selection (\myalg)}, since it exploits the semantic knowledge (i.e., attributes) of seen concepts for the ZSFS problem.

%se\textbf{M}antic based zer\textbf{O} sh\textbf{O}t featu\textbf{R}e s\textbf{E}lection (MOORE)
%as \emph{Semantic based Zero Shot Feature Selection (SZSFS)}, since we exploit the semantic knowledge of seen classes for the ZSFS problem.

%Note that our method can be extended to handle both seen and unseen concepts, if we (just like the traditional FS methods) incorporate the original class labels into the final objective function.
%We leave this extension as future work.
%into our model. incorporate
%consider the effect of the original label information as traditional feature selection methods do.

%if the effect of the original label information is also considered, which has been extensively studied by traditional feature selections.
%once we consider the effects of the original label information, which has been extensively studied by traditional feature selections.
%\textcolor[rgb]{1.00,0.00,0.00}{simultaneously consider the functional objectives} used in traditional supervised feature selection methods.
%consider the objective functions used in the existing traditional supervised feature selection methods.


\subsection{Optimization}
The optimization problem in Eq.~\ref{eq_final_cost01} is a `0/1' integer programming problem, which might be hard to solve by conventional optimization tools.
Therefore, in this subsection, we give an efficient solution for this problem.
%which is well known to be NP-hard~\cite{nemhauser1988integer}.
%First of all, to make the optimization tractable, we relax the `0/1' constraint on $s$ and only require $s$ to be non-negative.
First of all, to make the optimization tractable, we relax this `0/1' constraint by allowing $s$ to take real non-negative values.
%to be a non-negative real-valued.
% on $s$ and only require $s$ to be non-negative.
This relaxation yields the following optimization problem:
%\begin{equation}
%\small
%\label{eq_final_cost_relax}
%\begin{aligned}
%\underset{W, s}{\text{min }} & \mathcal{J} {=} \left \| Y_{s}{-}X\mathrm{diag}(s)W \right \|^{2}_{F} {+} \alpha \left \| Y_{s}{-}\bar{X}\mathrm{diag}(s)W \right \|^{2}_{F} {+} \gamma \left \| W \right \|^{2}_{F} \\
%\mathrm{s.t.}   & \hspace{0.5em} s \geq 0
%\end{aligned}
%\end{equation}
\begin{equation}
\small
\label{eq_final_cost_relax}
\begin{aligned}
\underset{W, s\geq 0}{\text{min }} & \mathcal{J} = \left \| Y_{s}{-}X\mathrm{diag}(s)W \right \|^{2}_{F} {+} \alpha \left \| Y_{s}{-}\bar{X}\mathrm{diag}(s)W \right \|^{2}_{F} \\
& \hspace{2em} + \gamma \left \| W \right \|^{2}_{F} \\
%\mathrm{s.t.}   & \hspace{0.5em} s \geq 0
\end{aligned}
\end{equation}

As such, the objective function is differentiable w.r.t. the real-valued $s$.
Intuitively, the value of $s_{i}$ can be interpreted as the importance score of $i$-th feature, i.e., important features would have higher scores, while the scores of unimportant features tend to shrink towards 0.
%Therefore, after obtaining the solution of Eq.~\ref{eq_final_cost_relax}, we can rank $s$ to identify important features.
%we can get the top ranked features.
%we can select features by solving this optimization problem.

%After obtaining the relaxed solution on $s$, we can get important features.
%rank all features according to the value of $s_{i}$  in a descending order and get the top ranked features.
%the feature selection for seen categories,
% to deal with applications to a wide variety of feature selection problems
%once we involve the loss term used in traditional supervised feature selection methods.


The optimization problem in Eq.~\ref{eq_final_cost_relax} can be solved iteratively.
%we adopt an alternating optimization framework to obtain a local optima
Specifically, this consists of the following two steps.

\paragraph{Fix $s$ and update $W$}
When $s$ is fixed, Eq.~\ref{eq_final_cost_relax} is convex w.r.t. $W$.
%Therefore, we remove the terms that are irrelevant to $W$, then reformulate the objective function in Eq.~\ref{eq_final_cost_relax} as follows:
Therefore, after removing the terms that are irrelevant to $W$, we can reformulate the objective function in Eq.~\ref{eq_final_cost_relax} as the following unconstrained optimization problem:

%\begin{equation}
%\small
%\label{eq_cost_relax_W}
%\begin{aligned}
%\underset{W}{\text{min }} & \mathcal{J}_{W} {=} \left \| Y_{s}{-}X\mathrm{diag}(s)W \right \|^{2}_{F} {+} \alpha \left \| Y_{s}{-}\bar{X}\mathrm{diag}(s)W \right \|^{2}_{F} {+} \gamma \left \| W \right \|^{2}_{F}
%\end{aligned}
%\end{equation}

\begin{equation}
\small
\label{eq_cost_relax_W}
\begin{aligned}
\underset{W}{\text{min }} & \mathcal{J}_{W} {=} \left \| Y_{s}{-}X\mathrm{diag}(s)W \right \|^{2}_{F} {+} \alpha \left \| Y_{s}{-}\bar{X}\mathrm{diag}(s)W \right \|^{2}_{F} \\
& \hspace{2em} + \gamma \left \| W \right \|^{2}_{F}
\end{aligned}
\end{equation}

By comparing the derivative of $\mathcal{J}_{W}$ w.r.t. $W$ to 0, we obtain the update solution for $W$:

%When $s$ if fixed, the derivations of Eq.~\ref{eq_final_cost_relax} with respect to $W$ is:
The derivative of $\mathcal{J}_{W}$ w.r.t. $W$ is:
\begin{equation}
\small
\label{eq_derive_W}
\begin{aligned}
&\frac{\partial \mathcal{J}_{W}}{\partial W} = -2(X\mathrm{diag}(s))'Y_{s} + 2(X\mathrm{diag}(s))'(X\mathrm{diag}(s))W\\
 &-2\alpha(\bar{X}\mathrm{diag}(s))'Y_{s} {+} 2\alpha(\bar{X}\mathrm{diag}(s))'(\bar{X}\mathrm{diag}(s))W {+} 2\gamma W\\
%&\frac{\partial \mathcal{J}}{\partial W} = -2(X\mathrm{diag}(s))'Y_{s} + 2(X\mathrm{diag}(s))'(X\mathrm{diag}(s))W\\
% &-2\alpha(B\mathrm{diag}(s))'Y_{s} + 2\alpha(B\mathrm{diag}(s))'(B\mathrm{diag}(s))W + 2\gamma W\\
% &\frac{\partial \mathcal{J}}{\partial W} = -2(XS)'Y_{s} + 2(XS)'(XS)W \\& -2\alpha(BS)'Y_{s} + 2\alpha(BS)'(BS)W + 2\gamma W \\
%& W = [(XS)'(XS) + \alpha (BS)'(BS) + \gamma I_{d}]^{-1}[(XS)' + \alpha (BS)']Y_{s}
\end{aligned}
\end{equation}
%
%\noindent By setting this derivative to zero, we obtain the closed form solution for $W$:
\begin{equation}
\small
\label{eq_update_W}
\begin{aligned}
%W =& [(XS)'(XS) {+} \alpha (\bar{X}S)'(\bar{X}S) {+} \gamma I_{d}]^{-1}[(XS)' {+} \alpha (\bar{X}S)']Y_{s} \\
W {=}& [(X\mathrm{diag}(s))'(X\mathrm{diag}(s)) {+} \alpha (\bar{X}\mathrm{diag}(s))'(\bar{X}\mathrm{diag}(s)) \\
& {+} \gamma I_{d}]^{-1}[(X\mathrm{diag}(s))' {+} \alpha (\bar{X}\mathrm{diag}(s))']Y_{s}
\end{aligned}
\end{equation}
%\subsubsection*{Fix $s$, $V$ and update $W$}
%The derivations of $\mathcal{J}$ with respect to $W$ is:
%\begin{equation}
%\label{eq_update}
%\begin{aligned}
%&\frac{\partial \mathcal{J}}{\partial W} = -2\alpha(X\mathrm{diag}(s))'Y_{s} + 2\alpha(X\mathrm{diag}(s))'(X\mathrm{diag}(s))W + 2\gamma W\\
%& W = [\alpha (X\mathrm{diag}(s))'(X\mathrm{diag}(s)) + \gamma I_{d}]^{-1}(\alpha X\mathrm{diag}(s))'Y_{s}
%\end{aligned}
%\end{equation}

\paragraph{Fix $W$ and update $s$}
When $W$ is fixed, the objective function in Eq.~\ref{eq_final_cost_relax} can be rewritten as follows:
%w.r.t. $s$ becomes:
\begin{equation}
\small
\label{eq_cost_relaxed_s}
\begin{aligned}
\underset{s\geq 0}{\text{min }} & \mathcal{J}_{s} {=} \left \| Y_{s}{-}X\mathrm{diag}(s)W \right \|^{2}_{F} {+} \alpha \left \| Y_{s}{-}\bar{X}\mathrm{diag}(s)W \right \|^{2}_{F}\\
%\mathrm{s.t.}   & \hspace{0.5em} s \geq 0
\end{aligned}
\end{equation}

%\begin{equation}
%\label{eq_obj_cost_s}
%\begin{aligned}
%\underset{s}{\text{min }} & \mathcal{J} = \left \| Y_{s}-X\mathrm{diag}(s)W \right \|^{2}_{F} + \alpha \left \| Y_{s}-B\mathrm{diag}(s)W \right \|^{2}_{F}  \\
%\mathrm{s.t.}   & \hspace{0.5em} s \geq 0
%\end{aligned}
%\end{equation}

%When $W$ is fixed, the derivations of Eq.~\ref{eq_final_cost_relax} with respect to $s$ is:
\noindent The derivative of $\mathcal{J}_{s}$ w.r.t. $s$ is:
\begin{equation}
\small
\label{eq_update_s}
\begin{aligned}
%\frac{\partial \mathcal{J}}{\partial s} = [- 2 X'Y_{s}W' + 2 X'XSWW' \\ -2\alpha B'Y_{s}W' + 2\alpha B'BSWW' ]_{pp}\\
%\frac{\partial \mathcal{J}}{\partial s} = [- 2 X'Y_{s}W' + 2 X'XSWW' \\ -2\alpha \bar{X}'Y_{s}W' + 2\alpha \bar{X}'\bar{X}SWW' ]_{pp}\\
\frac{\partial \mathcal{J}_{s}}{\partial s} &= [- 2 X'Y_{s}W' + 2 X'X\mathrm{diag}(s)WW' \\
& -2\alpha \bar{X}'Y_{s}W' + 2\alpha \bar{X}'\bar{X}\mathrm{diag}(s)WW' ]_{diag}\\
\end{aligned}
\end{equation}
where $[ \cdot ]_{diag}$ denotes the vector of diagonal elements of matrix $[\cdot]$.
% the diagonal element of matrix $[\cdot]$.
In addition, since we require $s$ to be non-negative, we perform Projected Gradient Descent (PGD)~\cite{calamai1987projected} for this constrained optimization problem.
Specifically, we project $s$ as $s = max(0, s)$ after each gradient updating step.
%Specifically, we project every $s$ as $s_{i} = max(0, s_{i}), \forall i=1,...,d$ after each gradient updating step.
%Specifically, we project $s$ to be non-negative after each gradient updating step:
%\begin{equation}
%\label{eq_project_s}
%\begin{aligned}
%\mathrm{Proj}(s_{i}) = max(0, s_{i}), \forall i=1,...,d
%\end{aligned}
%\end{equation}

%In sum, we can alternatively perform the above two steps until it converges or reaches user-specified maximum number of iterations.
In summary, we can alternatively perform the above two steps until it converges or reaches a user-specified maximum iteration number.
% the user-specified maximum iteration number
For clarity, we summarize this optimization procedure in Alg.~\ref{alg_ours}.

%Specifically, we project s back to [0 , 1] after each gradient updating step.
%$$s = max(0, s)$$

%\input{our_method_L1_center_x_center}



==> our_method_L1_center_x_center.tex <==
\section{Center - Feature Selection}
\begin{equation}
\label{eq_final_cost}
\begin{aligned}
\underset{W, s}{\text{min }} & \mathcal{J} = \left \| Xdiag(s) -Bdiag(s) \right \|^{2}_{F} \\
\mathrm{s.t.}   & \hspace{0.5em} s \in \{0,1\},\ s^{T}1_{d}=k
\end{aligned}
\end{equation}
where $W \in R^{d \times a}$ . \\

\textbf{Final:}
\begin{equation}
\label{eq_final_cost}
\begin{aligned}
\underset{s, W, V}{\text{min }} & \mathcal{J} = \left \| Y_{s}-Xdiag(s)W \right \|^{2}_{F} + \alpha \left \| Xdiag(s) -Bdiag(s) \right \|^{2}_{F}  + \gamma \left \| W \right \|^{2}_{F} \\
\mathrm{s.t.}   & \hspace{0.5em} s \in \{0,1\},\ s^{T}1_{d}=k
\end{aligned}
\end{equation}

\subsubsection*{Fix $s$ and update $W$}
The derivations of $\mathcal{J}$ with respect to $W$ is:
\begin{equation}
\label{eq_update}
\begin{aligned}
&\frac{\partial \mathcal{J}}{\partial W} = -2(XS)'Y_{s} + 2(XS)'(XS)W + 2\gamma W\\
& W = [ (XS)'(XS) + \gamma I_{d}]^{-1}( XS)'Y_{s}
\end{aligned}
\end{equation}

\subsubsection*{Fix $W$ and update $s$}
\begin{equation}
\label{eq_final_cost}
\begin{aligned}
\underset{W,s,v}{\text{min }} & \mathcal{J} = \left \| Y_{s}-Xdiag(s)W \right \|^{2}_{F} + \alpha \left \| Xdiag(s) -Bdiag(s) \right \|^{2}_{F}  \\
\mathrm{s.t.}   & \hspace{0.5em} s\geq 0
\end{aligned}
\end{equation}


The derivations of $\mathcal{J}$ with respect to $s$ is:
\begin{equation}
\label{eq_update}
\begin{aligned}
%\frac{\partial \mathcal{J}}{\partial s} = [-2X'Y_{s}W' + 2X'Xdiag(s)WW' \\- 2\alpha X'Y_{b}V' + 2\alpha X'Xdiag(s)VV']_{pp}\\
\frac{\partial \mathcal{J}}{\partial s} = [- 2 X'Y_{s}W' + 2 X'XSWW' \\
+2\alpha X'XS - 2\alpha (B'X + X'B)S + 2\alpha B'BS]_{pp}\\
\end{aligned}
\end{equation} 

==> our_method_gaussian.tex <==

%\input{preliminary_problem}
\section{The Proposed Method}
\subsection{Zero-Shot Feature Selection}
\begin{equation}
\label{eq_final_cost}
\begin{aligned}
& \underset{W}{\text{min}} & & \mathcal{J} = \left \| Y_{s}-XW \right \|^{2}_{F} + \gamma \left \| W \right \|_{21}
\end{aligned}
\end{equation}
where $W \in R^{d \times k}$ .
The L21-norm regularization term is imposed on $W$ to ensure that $W$ is sparse in rows, i.e., it achieves joint feature sparsity for all c latent semantic variables.

\begin{equation}
\label{eq_final_cost}
\begin{aligned}
& \underset{W}{\text{min}} & & \mathcal{J} = \left \| Y_{s}-XW \right \|^{2}_{F} + \gamma Tr(W^{T}DW)
\end{aligned}
\end{equation}
where $D$ is a diagonal matrix with the $i$-th diagonal element as:
$$D(i,i) = \frac{1}{2\left \| W(i,:) \right \|_{2} }$$

The derivations of $\mathcal{J}$ with respect to $W$ are:
\begin{equation}
\label{eq_update}
\begin{aligned}
&\frac{\partial \mathcal{J}}{\partial W} = -2X'Y_{s} + 2X'XW +2\gamma DW
\end{aligned}
\end{equation}


\subsection{Gaussian add}
We replace the Euclidean distance in our work by a learned (squared) Mahalanobis distance:

\begin{equation}
\label{eq_derive_W}
\begin{aligned}
D_{M}(Y_{s}(i,:), f(x_{i})) &= (Y_{s}(i,:) - f(x_{i})) M (Y_{s}(i,:) - f(x_{i}))' \\
& = (Y_{s}(i,:) - f(x_{i})) VV' (Y_{s}(i,:) - f(x_{i}))' \\
& = \left \| Y_{s}(i,:)V - f(x_{i})V \right \|^{2}_{F} \\
\end{aligned}
\end{equation}

In the above, we assume $M = VV'$, i.e., matrix $M$ can be factorized as two matrices.


%\begin{equation}
%\label{eq_final_cost}
%\begin{aligned}
%\underset{W, \sigma}{\text{min\ }} & \mathcal{J} = \left \| Y_{s}V{-}XWV \right \|^{2}_{F} + \gamma \left \| W \right \|_{21} \\
%\mathrm{s.t.}   & \hspace{0.5em} \left \| V \right \|^{2}_{F} = C\\
%\underset{W, \sigma}{\text{min\ }} & \mathcal{J} = \left \| Y_{s}V{-}XWV \right \|^{2}_{F} + \gamma \left \| W \right \|_{21} + \lambda (\left \| V \right \|^{2}_{F}-C) \\
%\end{aligned}
%\end{equation}

\begin{equation}
\label{eq_final_cost}
\begin{aligned}
\underset{W, V}{\text{min\ }} & \mathcal{J} = \left \| Y_{s}V{-}XWV \right \|^{2}_{F} + \gamma \left \| W \right \|_{21} \\
\mathrm{s.t.}   & \hspace{0.5em} V'V = I^{l\times l} \\
\end{aligned}
\end{equation}




\subsection{Optimization}

\subsubsection*{Fix $V$ and update $W$}
\begin{equation}
\label{eq_final_cost}
\begin{aligned}
& \underset{W}{\text{min}} & & \mathcal{J} = \left \| Y_{s}V-XWV \right \|^{2}_{F} + \gamma Tr(W^{T}DW)
\end{aligned}
\end{equation}

The derivations of $\mathcal{J}$ with respect to $W$ are:
\begin{equation}
\label{eq_update}
\begin{aligned}
&\frac{\partial \mathcal{J}}{\partial W} = -2X'Y_{s}VV' + 2X'XWVV' + 2\gamma DW
%&
\end{aligned}
\end{equation}

\subsubsection*{Fix $W$ and update $V$}

\begin{equation}
\label{eq_final_cost}
\begin{aligned}
\underset{W, L}{\text{min\ }} & \mathcal{J} = \left \| Y_{s}V{-}XWV \right \|^{2}_{F} \\
\mathrm{s.t.}   & \hspace{0.5em} V'V = I^{l\times l} \\
\end{aligned}
\end{equation}


We set $A=XW$.
\begin{equation}
\label{eq_derive_W}
\begin{aligned}
\mathcal{J} &= Tr( (YV-AV)'(YV-AV) ) \\
& = Tr( V'(Y-A)'(Y-A)V ) \\
\end{aligned}
\end{equation}

The optimal solution of $V$ are the eigenvectors corresponding to the $l$ smallest eigenvalues of $(Y-A)'(Y-A)$.

we can consider~\cite{xiang2008learning}.

$(Y-A)'(Y-A)$ must be positive semi-definite.


\section{The Proposed Method}\label{sect_method}
%In this section, we provide the detail
In this section, we provide a complete description of the proposed \myalg\ method.
%In this section, we provide details about the proposed \myalg\ method.
Firstly, we discuss the feasibility of transferring knowledge for newly-emerging instances from unseen classes.
Then, we describe the formulation of \myalg\ method.
Finally, we we provide an effective solution to address the optimization issue of \myalg.
%Finally, we analyse the computational complexity of the optimization method.

%In this section, we present the proposed ranking based
%factorization method for POI recommendation. We first
%formulate the POI recommendation problem by a ranking
%objective function, and then introduce how to optimize it.
%Finally, we generalize the model for time-aware POI recommendation.

\subsection{Transfer Knowledge for Unseen Classes}
%As mentioned above, the key idea is to reuse the supervised knowledge of seen classes for the coming unseen classes.
%On the other hand, class labels usually have semantic meanings, like ``cat'' and ``dog''.
%According to theory of ZSL, seen class labels can be described via semantic descriptions xxxx.
%Therefore, we can build vectorial representations in the semantic space for class labels which reflects the semantic relationship between them, i.e., the attributes describing the xxxxx. knowledge base of semantic properties
%In light of this,
%Based on this fact, the features, which best distinguish these attributes, could .
According to the theory of ZSL, the capacity of inferring attributes allows us to describe, compare, or even categorize unseen objects.
Take the seen classes in Fig.~\ref{fig_example} as an example, with the training images of these classes, we could learn a mapping function between image features and attributes (e.g., ``has stripes'', ``can fly'' and ``is metal'').
%learn a mapping function between low-level features and some attribute
% can learn the knowledge about some attributes (e.g., ``has stripes'', ``has fur'' or ``is metal'').
%We capture the knowledge about some attributes
%the attributes is captured
%With this learned knowledge, we can classify the unseen ``koala'' and ``helicopter'' by inferring their attributes without any training images.
%To recognize unseen object such as ``koala'' and ``helicopter'', we can use the learned knowledge to infer the attributes predict the attributes of the images
%With this learned knowledge,
As such, we can infer the attributes of the objects belonging to unseen classes such as ``koala'' and ``quadrotor'', so as to classify them without any training examples.
%In other words, ZSL approaches take attributes as an intermediate bridge to transfer knowledge from seen classes to unseen classes.

%At the testing stage, after successfully inferring the attributes of the unseen images, we can classify unseen classes such as ``koala'' and ``helicopter'' without any training images.
%With this learned knowledge, we can infer the attributes of unseen class ``koala'' and ``helicopter'', so as to classify them without any training images.

%In light of this, we use attribute representation to replace with the original independent binary label information.
%In light of this, as illustrated in Fig.~\ref{fig_example}, we project the original binary labels to semantic representation space.
In light of this, as illustrated in Fig.~\ref{fig_example}, we propose to replace the original class labels with attribute labels to guide feature selection.
%we use attribute labels to replace the original labels, so as to further guide feature selection.
Compared to the original class labels, attribute labels not only reflect the differences among seen classes but also provide additional semantic information about the unseen classes.
% discriminative information
%In this way, supervised knowledge are successfully transferred from the seen classes to unseen classes.
In other words, by introducing attribute labels, we can transfer the supervised knowledge from the seen classes to unseen classes.
% by these attribute labels.
%After that, feature selection is guided by these attributes.
%Since these attributes provide discriminative semantic descriptions about the unseen categories, the selected features should also have this discriminative power.
%use attribute representation to replace with the original independent binary label information.
%Specifically, for each seen class type, we replace the original binary labels with its attribute representation vector.
%In this semantic space, semantic correlations among different classes can be quantitatively measured and captured.
%These attributes provide semantic information about the unseen categories.
%Every class label is described by pure text.
%In the subsequent part, we denote the used semantic attribute labels as $Y_{s} {\in} \mathbb{R}^{n, a}$, where $a$ is the attribute number.
In the subsequent part, we denote this kind of semantic labels as $Y_{s} {\in} \mathbb{R}^{n \times a}$, where $a$ is the attribute number.
These attribute labels can either be provided manually or generated automatically from online textual documents~\cite{rohrbach2010helps}, such as Wikipedia articles.
%In other words, each seen class is described by a xxxxxx.~\cite{qiao2016less}
%With these Then we can select features best
%After that, if we can select the features which best distinguish these attributes.
%Since these attributes provide semantic information about the unseen categories, with these attributes, the selected features should also have this generalizing power.
%Since these attributes have the capability to distinguish the coming unseen classes, the selected features should also have this generalizing power.
%When an unseen object shows up, these attribute discriminative features are capable to categorize unseen objects in a semantic level.
%When learning the attributes, we could generalize to new types of objects
%the seen class labels can be projected into the semantic space.
%This is because attributes are shared across different categories and provide a compact but discriminative representation.
%Therefore, unseen labels can
%leverage the well-established mapping from its semantically close
%seen categories.
%In this paper, we adopt pure textual descriptions as attributes to describe seen class labels.
%These attributes can either be manually given or .

\subsection{Zero-Shot Feature Selection}
\subsubsection*{Feature selection with attribute labels}
%With the used semantic labels, the feature selection procedure is described as follows.
%we can perform feature selection.
%Recall that we intend to use the amendatory supervised knowledge to guide the feature selection $Y_{s}$.
We use $s {=} \{0, 1\}^{d}$ as the indicator vector, where $s_{i} $=$ 1$ if the $i$-th feature is selected and $s_{i} $=$ 0$ otherwise.
%Let us denote the diagonal matrix with diagonal elements $s$ as $diag(s)$.
%Diag(s) denotes the matrix with the main diagonal beings
Denote $\mathrm{diag}(s)$ as the matrix with the main diagonal being $s$, then the original data can be represented as $X\mathrm{diag}(s)$ with the selected features.
%Then, the original data can be represented as $X\mathrm{diag}(s)$ with the selected features.
%Therefore, the new representation of training example constructed by the selected features is $X\mathrm{diag}(s)$.
%Therefore, the selected features comprise a new representation of training example, and we denote it as $X\mathrm{diag}(s)$.
% can be represented as $ X' = X\mathrm{diag}(s)$.
From a generative point of view, we assume that the selected features could generate the given attribute labels.
%We further assume that these selected features could generate the amendatory supervised knowledge $Y_{s}$.
For simplicity and efficiency, we use a linear generating function $W\in R^{d \times a}$, and adopt the squared loss to measure the error.
%Then the generation can be captured by the following optimization problem:
Therefore, the optimal $s$ is given by the following optimization problem:
%Thus, the feature selection problem can be captured by the following optimization problem:
%Recall that we intend to use the amendatory supervised knowledge to guide the feature selection $Y_{s}$, the generation can be captured by the following optimization problem:
%\begin{equation}
%\label{eq_basic_source}
%\begin{aligned}
%\underset{f}{\text{min }} & \sum_{i=1}^{n_{s}}\mathcal{L}(f(x_{i}\mathrm{diag}(s)),y_{si}) + \mathcal{R}(f) \\
%\mathrm{s.t.}   & \hspace{0.5em} s \in \{0,1\},\ s^{T}1_{d}=k
%\end{aligned}
%\end{equation}
%where $\mathcal{L}(\cdot,\cdot)$ is a loss function, $f$ is the learned classifier, and $\mathcal{R}$ is the regularization term for $f$ to avoid overfitting.



\begin{equation}
\label{eq_semantic_selection}
\begin{aligned}
\underset{W, s}{\text{min }} & \mathcal{J}_{1} = \left \| Y_{s}-X\mathrm{diag}(s)W \right \|^{2}_{F} + \gamma \left \| W \right \|^{2}_{F} \\
\mathrm{s.t.}   & \hspace{0.5em} s \in \{0,1\}^{d},\ s^{T}1_{d}=k
\end{aligned}
\end{equation}
where $k$ is the number of features to select, and $\gamma$ is the regularization parameter to avoid overfitting.
%The benefit of the above formulation is that it can narrow down the semantic gap between seen and unseen classes.
The benefit of the above approach is that the selected features capture the discriminative power of categorizing unseen objects via attributes.

%Problem~\ref{eq_semantic_selection} can be seen as the classical ($\ell_{1}$-norm based) Lasso problem with the modified supervised knowledge.
%By finding the solution that minimize Eq.~\ref{eq_semantic_selection}, we select $k$ features which best generate semantic labels (descriptions) of seen classes.
%select features that are beneficial in learning attribute classifiers.
%We can even learn new categories withnovisual examples, using textual de-scriptions instead.

\subsubsection*{The center-characteristic loss}
%\begin{figure}[htbp]
%\centering
%    \includegraphics[width=0.4\textwidth]{images/center_loss.pdf}
%\caption{Separable Features vs. Discriminative Features (center loss) \protect\cite{wen2016discriminative}.}
%\label{fig_center-loss}
%\end{figure}

\begin{figure}[!t]
\centering
    \includegraphics[width=0.5\textwidth]{images/center_character_loss.pdf}
%\caption{Center loss \protect\cite{wen2016discriminative} vs. center-characteristic loss.}
\caption{Center loss vs. Center-characteristic loss.}
\label{fig_center-loss}
\end{figure}


Recent work of supervised feature learning~\cite{wen2016discriminative}, i.e., \emph{center loss}, has pointed out that discriminative features are more generalized for identifying unseen objects than separable features.
Specifically, as illustrated in Fig.~\ref{fig_center-loss}, center loss minimizes the distances between the learned features and their corresponding class centers.
%has pointed out that the learned features should close to their corresponding class centers
%The learned features need to be not only separable but also discriminative...
%generalized enough for identifying new unseen
%As illustrated in Fig.~\ref{fig_center-loss}, discriminative features better compact intra-class variations and distinguish inter-class differences.
%As shown in Fig.~\ref{fig_center-loss}, discriminative features better compact intra-class variations and distinguish inter-class differences.
%Motivated by this, we force the the selected features should be close to their corresponding class centers.
%Accordingly, we minimize the distances between the selected features and their corresponding class centers, which yields the following minimization problem:
Accordingly, for the feature selection task, it minimizes the distances between the selected features and their corresponding class centers, which yields the following minimization problem:
%by minimizing the following objective function.
%encourage to select the features lying close to their corresponding class centers.
%This minimizes the following objective function:
%we introduce a new loss function for feature selection, \emph{self-centeredness loss}, namely the selected features should be close to their corresponding class centers.
\begin{equation}
\label{eq_center-loss}
\begin{aligned}
\underset{s}{\text{min }} & \mathcal{J}_{2} = \left \| X\mathrm{diag}(s) -\bar{X}\mathrm{diag}(s) \right \|^{2}_{F} \\
%\sum_{i=1}^{n}\left \| x_{i}\mathrm{diag}(s) -\bar{x}_{i}\mathrm{diag}(s) \right \|^{2}_{F} \\
\mathrm{s.t.}   & \hspace{0.5em} s \in \{0,1\}^{d},\ s^{T}1_{d}=k
\end{aligned}
\end{equation}
%where $\bar{x}_{i}$ is the denotes the $y_{i}$-th class center of features.
where $\bar{X} = \{\bar{x}_{1}, ..., \bar{x}_{n} \}'\in \mathbb{R}^{n \times d}$, and $\bar{x}_{i}$ denotes the feature vector of the $y_{i}$-th class center.
%$\bar{x}_{i}$ denotes the $y_{i}$-th class center of features.

However, this constraint may be too harsh for a feature selection task, since all features are pre-extracted.
Therefore, we modify this constraint by multiplying the terms in the square loss with the generating function $W$, as XXXXXXXXXX for some reasons.
and approximate $X\mathrm{diag}(s)W$ with $Y_{s}$ according to Eq.~\ref{eq_semantic_selection}.
%Finally, we get the following loss function:
After this modification, Eq.~\ref{eq_center-loss} becomes:
\begin{equation}
\label{eq_self-center-loss}
\begin{aligned}
\underset{W,s}{\text{min }} & \mathcal{J}_{2} = \left \| Y_{s}-\bar{X}\mathrm{diag}(s)W \right \|^{2}_{F}  \\
\mathrm{s.t.}   & \hspace{0.5em} s \in \{0,1\}^{d},\ s^{T}1_{d}=k
\end{aligned}
\end{equation}

We call this loss function \emph{center-characteristic loss}, as it encourages the selected features to capture the central characteristics of seen classes' attributes (illustrated in Fig.~\ref{fig_center-loss}).
Meanwhile, xxxx to attributes.
Intuitively, this xxxx aims to.
%compacts intra-class variations
%it encourages the selected features to lie in
% encourages diversity between individual predictors of an ensemble
%compact intra-class variations
%namely for each class, the selected feature should close to the class center.
%%Intuitively, this loss function ensures the selected features should lie in the cluster centers.
%Intuitively, the features which capture the central characteristics of seen classes are preferred.


%namely the selected features should not only separable but also discriminative.
%In other words, the selected feature should tend to self-centeredness.
%Feature center loss should show lower intra-class variations.

\subsubsection*{Zero-Shot feature selection framework}
By combining the objective functions in Eqs.~\ref{eq_semantic_selection} and~\ref{eq_self-center-loss}, the proposed method ZSFS is to solve the following optimization problem:
%\textbf{Final:}
\begin{equation}
\small
\label{eq_final_cost01}
\begin{aligned}
\underset{W, s}{\text{min }} & \mathcal{J} {=} \left \| Y_{s}{-}X\mathrm{diag}(s)W \right \|^{2}_{F} {+} \alpha \left \| Y_{s}{-}\bar{X}\mathrm{diag}(s)W \right \|^{2}_{F} {+} \gamma \left \| W \right \|^{2}_{F} \\
\mathrm{s.t.}   & \hspace{0.5em} s \in \{0,1\}^{d},\ s^{T}1_{d}=k
\end{aligned}
\end{equation}
where $\alpha$ is a balancing parameter.
Note that our method can be extended to handle both seen and unseen classes, if we, just like the traditional feature selection methods, incorporate the original class label information into the final objective function.
%into our model. incorporate
%consider the effect of the original label information as traditional feature selection methods do.

%if the effect of the original label information is also considered, which has been extensively studied by traditional feature selections.
%once we consider the effects of the original label information, which has been extensively studied by traditional feature selections.
%\textcolor[rgb]{1.00,0.00,0.00}{simultaneously consider the functional objectives} used in traditional supervised feature selection methods.
%consider the objective functions used in the existing traditional supervised feature selection methods.


\subsection{Optimization}
The optimization problem in Eq.~\ref{eq_final_cost01} is a `0/1' integer programming problem, which might be hard to solve by existing optimization tools.
Therefore, in this subsection, we give an efficient solution for this problem.
%which is well known to be NP-hard~\cite{nemhauser1988integer}.
Specifically, to make the optimization tractable, we relax the `0/1' constraint on $s$ and only require $s$ to be non-negative.
This relaxation yields the following optimization problem:
\begin{equation}
\small
\label{eq_final_cost_relax}
\begin{aligned}
\underset{W, s}{\text{min }} & \mathcal{J} {=} \left \| Y_{s}{-}X\mathrm{diag}(s)W \right \|^{2}_{F} {+} \alpha \left \| Y_{s}{-}\bar{X}\mathrm{diag}(s)W \right \|^{2}_{F} {+} \gamma \left \| W \right \|^{2}_{F} \\
\mathrm{s.t.}   & \hspace{0.5em} s \geq 0
\end{aligned}
\end{equation}

The value of $s_{i}$ can be interpreted as the importance score of $i$-th feature.
Important features would have higher scores, while the scores of unimportant features tend to shrink towards 0.
Therefore, after obtaining the solution of Eq.~\ref{eq_final_cost_relax}, we can get the top ranked features.
%we can select features by solving this optimization problem.

%After obtaining the relaxed solution on $s$, we can get important features.
%rank all features according to the value of $s_{i}$  in a descending order and get the top ranked features.
%the feature selection for seen categories,
% to deal with applications to a wide variety of feature selection problems
%once we involve the loss term used in traditional supervised feature selection methods.


The optimization problem in Eq.~\ref{eq_final_cost_relax} can be solved iteratively.
%we adopt an alternating optimization framework to obtain a local optima
Specifically, the optimization algorithm consists of the following two steps.

\subsubsection*{Fix $s$ and update $W$}
When $s$ if fixed, the derivations of Eq.~\ref{eq_final_cost_relax} with respect to $W$ is:
\begin{equation}
\label{eq_derive_W}
\begin{aligned}
&\frac{\partial \mathcal{J}}{\partial W} = -2(X\mathrm{diag}(s))'Y_{s} + 2(X\mathrm{diag}(s))'(X\mathrm{diag}(s))W\\
 &-2\alpha(\bar{X}\mathrm{diag}(s))'Y_{s} {+} 2\alpha(\bar{X}\mathrm{diag}(s))'(\bar{X}\mathrm{diag}(s))W {+} 2\gamma W\\
%&\frac{\partial \mathcal{J}}{\partial W} = -2(X\mathrm{diag}(s))'Y_{s} + 2(X\mathrm{diag}(s))'(X\mathrm{diag}(s))W\\
% &-2\alpha(B\mathrm{diag}(s))'Y_{s} + 2\alpha(B\mathrm{diag}(s))'(B\mathrm{diag}(s))W + 2\gamma W\\
% &\frac{\partial \mathcal{J}}{\partial W} = -2(XS)'Y_{s} + 2(XS)'(XS)W \\& -2\alpha(BS)'Y_{s} + 2\alpha(BS)'(BS)W + 2\gamma W \\
%& W = [(XS)'(XS) + \alpha (BS)'(BS) + \gamma I_{d}]^{-1}[(XS)' + \alpha (BS)']Y_{s}
\end{aligned}
\end{equation}

By setting this derivative to zero, we obtain the closed form solution for $W$:
\begin{equation}
\label{eq_update_W}
\begin{aligned}
%W =& [(XS)'(XS) {+} \alpha (\bar{X}S)'(\bar{X}S) {+} \gamma I_{d}]^{-1}[(XS)' {+} \alpha (\bar{X}S)']Y_{s} \\
W {=}& [(X\mathrm{diag}(s))'(X\mathrm{diag}(s)) {+} \alpha (\bar{X}\mathrm{diag}(s))'(\bar{X}\mathrm{diag}(s)) \\
& {+} \gamma I_{d}]^{-1}[(X\mathrm{diag}(s))' {+} \alpha (\bar{X}\mathrm{diag}(s))']Y_{s}
\end{aligned}
\end{equation}
%\subsubsection*{Fix $s$, $V$ and update $W$}
%The derivations of $\mathcal{J}$ with respect to $W$ is:
%\begin{equation}
%\label{eq_update}
%\begin{aligned}
%&\frac{\partial \mathcal{J}}{\partial W} = -2\alpha(X\mathrm{diag}(s))'Y_{s} + 2\alpha(X\mathrm{diag}(s))'(X\mathrm{diag}(s))W + 2\gamma W\\
%& W = [\alpha (X\mathrm{diag}(s))'(X\mathrm{diag}(s)) + \gamma I_{d}]^{-1}(\alpha X\mathrm{diag}(s))'Y_{s}
%\end{aligned}
%\end{equation}

\subsubsection*{Fix $W$ and update $s$}
%When $W$ is fixed, the objective function in Eq. 5 w.r.t. $s$ becomes:
%\begin{equation}
%\label{eq_obj_cost_s}
%\begin{aligned}
%\underset{W, s}{\text{min }} & \mathcal{J} {=} \left \| Y_{s}{-}X\mathrm{diag}(s)W \right \|^{2}_{F} {+} \alpha \left \| Y_{s}{-}\bar{X}\mathrm{diag}(s)W \right \|^{2}_{F}\\
%\mathrm{s.t.}   & \hspace{0.5em} s \geq 0
%\end{aligned}
%\end{equation}

%\begin{equation}
%\label{eq_obj_cost_s}
%\begin{aligned}
%\underset{s}{\text{min }} & \mathcal{J} = \left \| Y_{s}-X\mathrm{diag}(s)W \right \|^{2}_{F} + \alpha \left \| Y_{s}-B\mathrm{diag}(s)W \right \|^{2}_{F}  \\
%\mathrm{s.t.}   & \hspace{0.5em} s \geq 0
%\end{aligned}
%\end{equation}

When $W$ is fixed, the derivations of Eq.~\ref{eq_final_cost_relax} with respect to $s$ is:
\begin{equation}
\label{eq_update_s}
\begin{aligned}
%\frac{\partial \mathcal{J}}{\partial s} = [- 2 X'Y_{s}W' + 2 X'XSWW' \\ -2\alpha B'Y_{s}W' + 2\alpha B'BSWW' ]_{pp}\\
%\frac{\partial \mathcal{J}}{\partial s} = [- 2 X'Y_{s}W' + 2 X'XSWW' \\ -2\alpha \bar{X}'Y_{s}W' + 2\alpha \bar{X}'\bar{X}SWW' ]_{pp}\\
\frac{\partial \mathcal{J}}{\partial s} &= [- 2 X'Y_{s}W' + 2 X'X\mathrm{diag}(s)WW' \\
& -2\alpha \bar{X}'Y_{s}W' + 2\alpha \bar{X}'\bar{X}\mathrm{diag}(s)WW' ]_{diag}\\
\end{aligned}
\end{equation}
where $[ \cdot ]_{diag}$ denotes the vector of diagonal elements of matrix $[\cdot]$.
% the diagonal element of matrix $[\cdot]$.
In addition, since we require $s$ to be non-negative, we perform Projected Gradient Descent (PGD)~\cite{calamai1987projected} for this constrained optimization problem.
Specifically, we project $s$ as $s = max(0, s)$ after each gradient updating step.


In sum, we can alternatively perform the above two steps until it converges or reaches user-specified maximum number of iterations.
For clarity, we summarize this optimization approach in Alg.~\ref{alg_ours}.

%Specifically, we project s back to [0 , 1] after each gradient updating step.
%$$s = max(0, s)$$

%\input{our_method_L1_center_x_center}



==> preliminary.tex <==
%\section{PRELIMINARY}\label{section_problem_statement}
\begin{table}[ht]
\caption{NOTATIONS}
\centering
\begin{tabular}{c|l}
\hline
Symbol    & Description \\
\hline
$\mathcal{C}$, $\mathcal{C}^{u}$                                                   & seen and unseen class set \\
$X \in \mathbb{R}^{n\times d}$                                  & the $n$ seen images \\
$S \in \mathbb{R}^{a\times c}$                                  & the attribute matrix of seen classes \\
$W \in \mathbb{R}^{d\times r}$                                  & xxxx   \\
%$M \in R^{a \times a}$                                          & mahalanobis matrix   \\
%$V \in R^{a \times l}$                                          & low-rank matrix: $M = VV'$   \\
$Y \in \mathbb{R}^{n \times c}$                                 & the label indicator matrix of seen data\\
$Y_{s} \in \mathbb{R}^{n \times a}$                                 & the sematic indicator matrix of seen data\\
$s \in R^{d \times 1}$                                          & the selected features \\
$1 \in R^{d \times 1}$                                          & column vector with all 1s \\
\hline
\end{tabular}
\label{tab_notations}
\end{table} 

==> related_ijcai.tex <==
\section{Related Work}
\subsection{Feature Selection}
%Feature selection, which selects a proper subset of original features, plays an important role in the pattern recognition and machine learning areas.
%Feature selection (FS), which selects a subset of the original features according to some criteria, plays an important role in pattern recognition and machine learning areas.
Feature selection (FS) is a common and key problem in pattern recognition and machine learning areas.
%In terms of the label availability, existing feature selection methods can be roughly classified into two groups: unsupervised methods and supervised methods.
In terms of the label availability, existing FS methods can be roughly classified into three groups: unsupervised, supervised and semi-supervised FS methods.
%In unsupervised scenario, unsupervised methods~\cite{he2005laplacian,wang2014unsupervised}, tend to select the features best preserving the data similarity or manifold structure derived from the whole feature space.
In the unlabeled case, unsupervised methods select features which best keep the intrinsic structure of data according to various criteria, such as data variance~\cite{dash2000feature} and  data separability~\cite{cai2010unsupervised}.
%data similarity~\cite{nie2008trace} and data separability~\cite{cai2010unsupervised}.
%When no labeled data is available,
%In terms of the label availability, feature selection methods can be grouped into unsupervised methods or supervised methods.
%Unsupervised methods~\cite{he2005laplacian}~\cite{wang2014unsupervised}, which do not need any label information, tend to select the features best preserving the data similarity or manifold structure derived from the whole feature space.
%Supervised methods~\cite{cai2013exact,liu2013efficient} always assume that the whole dataset contains a fully labeled part and an unlabeled part.
%To take the advantage of labeled data, supervised methods~\cite{lee1988thirteen,cai2013exact} evaluate features by their correlation with the given class labels.
To take advantage of labeled data, supervised methods~\cite{cai2013exact} evaluate features by their relevance to the given class labels.
%Supervised methods~\cite{lee1988thirteen,cai2013exact} utilize the labeled data, and evaluate features by their correlation with the given class labels.
%assume some of the data must be labeled,
%and evaluate features by their correlation with the given class labels.
%assume that some data are labeled and others are unlabeled.
%The importance of a feature is then evaluated by its correlation with the given class labels.
%The higher correlation indicates a more important feature.
%The typical supervised methods include Pearson correlation coefficient~\cite{lee1988thirteen} and Fisher score~\cite{duda1995pattern}.
Extended from unsupervised and supervised methods, semi-supervised methods~\cite{kong2010semi} utilize both labeled and unlabeled data to mine the feature relevance.
%adopt both the labeled and unlabeled data to mine the feature
%relevance by assuming that the data lies on a low-dimensional
%manifold or is sampled from the same distribution
%
%utilize both labeled data and unlabeled data to learn the manifold
%structure [Lin and Zha 2008] [Zhu 2011] for feature selection.
%
%of the data samples with known class labels to provide prior knowledge for most data samples without
%class labels. Therefore it is a good compromise between supervised
%and unsupervised methods

%When label information is available, feature selection methods are either supervised or semi-supervised.
%%Supervised and Semi-supervised feature selection methods
%Supervised feature selection methods assume that some data are labeled and others are unlabeled.
%They then determine the importance of a feature by evaluating its correlation with the given class labels.
%The higher correlation indicates a more important feature.
%The typical supervised methods include Pearson correlation coefficient~\cite{lee1988thirteen} and Fisher score~\cite{duda1995pattern}.
%Semi-supervised methods~\cite{pierre2007semi,liu2013efficient} work in much the same way, except that they consider both labeled and unlabeled data together for feature selection.

%Existing work has demonstrated the effectiveness of these feature selection methods.
%However, they have a critical limitation: they require the training data and testing data belong to the same classes.
%%share the same concept.
%%require source and target domains have same classes.
%%they require the classes in source and target domains are the same.
%%In other words, the selected features can not discrimnit the images of unseen categories.
%In real-world applications, it is expected that we can also select the representative features for the images of unseen categories.
%Existing work fails to handle this problem.

It should be noted that traditional FS methods do not consider the generalization to ``unseen'' concepts, limiting in the ``seen'' area where every concept should at least provide one (unlabeled or labeled) instance.
%where every category should at least provide one training image.
In light of the knowledge explosion, with the rapid growth of newly-emerging concepts and multimedia data, building a FS model that generalizes well to unseen concepts has practical importance.
%Due to the rapid growth of newly-emerging concepts, building a FS model that generalizes well to unseen concepts has practical importance.
%is very important for real-world applications.
%a feature selection method which can perform well on unseen data is strongly needed.

\subsection{Attribute-based Zero Shot Learning}
%\subsection{Zero Shot Learning}
%Zero Shot Learning
%classifiers from seen classes and aims to classify the ob-jects of unseen classes
%Zero Shot Learning (ZSL)~\cite{lampert2009learning}~\cite{farhadi2009describing} aims to recognize unseen objects without training examples, by providing a high-level description of new classes that relate
%
%ZSL consists in recognising new categories of
%instances without training examples, by providing a high-level description of the new categories that relate them to
%categories previously learned by the machine.
%
%ZSL mainly is inherently a two stage process.
%It first learns the knowledge about the attributes,
%In the training stage, knowledge about the attributes is captured, and in the inference stage this
%knowledge is used to categorise instances among a new set
%of classes.
%
%It can thus be re-used for knowledge
%transfer between the source and target sets: the knowledge about the attributes is first captured, then this knowledge is used to categorise instances among a new set of classes.
%a projection
%function mapping low-level features to the semantic
%representation is learned from the auxiliary data by
%classifier or regressor. This projection is then applied to
%map each unlabelled target class instance into the same
%semantic space. In this space, a ‘prototype’ of each target
%class is specified, and each projected target instance is
%classified by measuring similarity to the class prototypes.
%
%Lampert et al. [12] adopted a set of attributes ob-tained from a psychology study. By learning probabilistic
%predictors of those attributes, they developed a framework
%to estimate the posterior of the test class.
The task of Zero Shot Learning (ZSL)~\cite{lampert2009learning,farhadi2009describing,akata2016multi} is to recognize unseen objects without any label information.
To achieve this goal, it leverages an intermediate semantic level (i.e., attribute layer) which is shared in both seen and unseen concepts.
%Taking the seen concepts in Fig.~\ref{fig_method} as an example, possible attributes include ``has stripes'', ``can fly'' and ``is metal''.
%In the training stage, the knowledge about these attributes (of seen concepts) is captured, and in the inference stage this knowledge is used to categorize instances among a set of unseen concepts.
%In the training stage, we could learn a mapping function between image features and these attributes of seen concepts.
%Then, we can
%In the inference stage, we can infer the same attributes of unseen
%the same attributes of the objects belonging to unseen concepts such as ``koala'' and ``quadrotor'', and then
%Finally, by computing the similarity between the test
%image’s attributes with each target class’ attributes
%Finally, the recognition result is obtained by comparing the recognized attributes of images with the class attributes.
Taking the seen concepts in Fig.~\ref{fig_method} as an example.
%We can define some attributes like ``has stripes'', ``can fly'' and ``is metal''.
We can define some attributes like ``can swim'', ``can fly'' and ``is metal''.
Then, we can train attribute recognizers using images and attribute information from seen concepts.
After that, given an image belonging to unseen concepts, these attribute recognizers can infer the attributes of this image.
Finally, the recognition result is obtained by comparing the test image's attributes with each unseen concept's attributes.

%In the inference stage, this knowledge is used to categorize instances among a set of unseen concepts by
%In the inference stage, this knowledge is used to categorize instances among a set of unseen concepts by
%
%In the inference stage, this knowledge is used to recognize the same attributes of unseen concepts, so as to categorize them.

%in instances from unseen concepts, so as to categorize these instances.
%the novel test categories

%a new set of concepts.

%The task of Zero Shot Learning (ZSL)~\cite{lampert2009learning,farhadi2009describing} is to recognize unseen objects without any label information.
%To achieve this goal, it leverages an intermediate semantic level (i.e., attribute layer) which is shared in both seen and unseen classes.
%Take the unseen class objects in Fig.~\ref{fig_example} as an example, possible attributes include ``has stripes'', ``can fly'' and ``is metal''.
%In the training stage, the knowledge about these attributes is captured, and in the inference stage this knowledge is used to categorise instances among a new set of classes.
%ZSL methods would capture the knowledge about these attributes based on the training instances of seen classes, and then use this knowledge to category instances among a new set of classes.
%Specifically, in the training stage, the knowledge about attributes is captured, and in the inference stage this knowledge is used to categorise instances among a new set of classes.
%it captures the knowledge about the attributes, and in the inference stage .
%knowledge about the attributes is captured, and in the inference stage this knowledge is used to categorise instances among a new set of classes.
%The key idea underpinning ZSL approaches is to transfer knowledge from seen classes to unseen classes via an intermediate-level
%semantic representation
%This can be done by means of leveraging an intermediate level: the at-tributes that provide semantic information about the cate-gories to classify.
%To achieve this goal, it transfers knowledge form seen classes to unseen classes by leveraging some high-level descriptions (i.e., attributes) shared between both seen and unseen classes.
%To achieve this goal, it adopts some high-level descriptions shared between these both seen and unseen classes, i.e., attributes, as the bridge for knowledge transfer.
%Take the seen objects in Fig.~\ref{fig_example} as an example, possible attributes include ``has stripes'', ``can fly'' and ``is metal''.
%These attributes not only provide semantic information about the unseen classes, but also
%
%To achieve this goal, it reuses already acquired label information by transferring knowledge from other related and well labeled seen categories.
%Specifically, some high-level descriptions, i.e., attributes, are used as the bridge for knowledge transfer.
%Take the seen objects in Fig.~\ref{fig_example} as an example, possible attributes include ``has stripes'', ``can swim'' or ``is metal''.
%These attributes can either be provided manually~\cite{farhadi2009describing} or automatically generated from unannotated text corpora~\cite{rohrbach2010helps,qiao2016less}.
%, such as Wikipedia articles

Although various ZSL methods have been proposed recently, they are mainly limited to classification or prediction applications.
%However, ZSL methods are mainly limited to classification or prediction applications.
To our best knowledge, this is the first study to consider the zero-shot setting in the FS problem.
%identify key features for novel images that were not observed.
%Our ZSFS enriches the family of zero-shot learning.
%In particular, we instead directly model the labels and are able to select useful features for unseen classes.


%Existing ZSL work mainly focus on the object recongigiation task.
%However, how to utilize the knowledge transferred from totally different classes to enhance feature selection is still an unexplored research issue.


==> result_classification.tex <==



\begin{table*}[htb]
\caption{Classification results on CIFAR10 dataset.}
\centering % used for centering table
\begin{tabular}{l|l|rrrrrrrrrr}
\hline
    &Method & 5 & 10 & 15 & 20 & 25 &30 &35 &40 &45 &50  \\
\hline
\multirow{7}{*}{Micro-F1(\%)} &
    Random          &0.3151    &0.3362    &0.3454    &0.3486    &0.356    &0.3626    &0.3694    &0.3861    &0.3931    &0.3984 \\
&   MCFS          &0.x    &0.2961    &0.3045    &0.3249    &0.3517    &0.3850    &0.4009    &0.4486    &0.4523    &0.4637 \\
&   FSASL15       &0.x    &0.2424    &0.2924    &0.3234    &0.3483    &0.3763    &0.3941    &0.3926    &0.4115    &0.4535 \\ %alpha=1
&   LASSO1        &0.x    &0.2503    &0.2503    &0.2506    &0.2507    &0.2507    &0.2506    &0.2506    &0.2506    &0.2506 \\
&   L20ALM     &0.x    &0.2356    &0.3132    &0.3302    &0.3483    &0.3336    &0.4459    &0.4179    &0.4266    &0.4705\\%巨慢
&   Our\_L1             &0.x    &0.3343    &0.4051    &0.4266    &0.4792    &0.5064    &0.5397    &0.5216    &0.5333    &0.5719 \\
&   Our\_L1\_center      &0.x    &0.3343    &0.4138    &0.4372    &0.4663    &0.5310    &0.5915    &0.5484    &0.5711    &0.5919 \\
&   Our        &0.x    &0.3604    &0.4826    &0.5023    &0.5064    &0.5450    &0.5261    &0.5753    &0.5828    &0.5930 \\
&   Our\_nor\_con    &0.x    &0.2995    &0.3563    &0.3918    &0.4459    &0.4750    &0.4773    &0.5378    &0.6097    &0.5934   \\
&   center\_semantic   &0.x    &0.3014    &0.3737    &0.4257    &0.4007    &0.4357    &0.4650    &0.4766    &0.4879    &0.5034 \\
&   center\_binary      &0.x    &0.2470    &0.2765    &0.3056    &0.3498    &0.3238    &0.3952    &0.3865    &0.4115    &0.4138 \\
&   Our\_L1\_s\_binary       &0.x    &0.3487    &0.3336    &0.4603    &0.4576    &0.4864    &0.4868    &0.4902    &0.5291    &0.5238 \\
&   LASSO0.1        &0.x    &0.2470    &0.2765    &0.3056    &0.3498    &0.3238    &0.3952    &0.3865    &0.4115    &0.4138    \\
&   Our\_L1\_center\_b        &0.x    &0.3487    &0.3336    &0.4603    &0.4576    &0.4864    &0.4868    &0.5008    &0.5291    &0.5238    \\
\hline
\multirow{7}{*}{Macro-F1(\%)} &
    Random          &0.2957    &0.3258    &0.3366    &0.3397    &0.3481    &0.3555    &0.3626    &0.3796    &0.3871    &0.3919 \\
%&   LapScore      &0.x    &0.1822    &0.2004    &0.2104    &0.2021    &0.2613    &0.2842    &0.2842    &0.2930    &0.2946  \\
&   MCFS          &0.x    &0.2780    &0.2881    &0.2899    &0.3428    &0.3800    &0.4062    &0.4309    &0.4399    &0.4550 \\
&   FSASL15        &0.x    &0.1420    &0.2124    &0.2431    &0.2746    &0.2921    &0.3275    &0.3230    &0.3494    &0.3893 \\
&   LASSO1        &0.x    &0.00027    &0.00029    &0.00058    &0.00063    &0.00070    &0.00057    &0.00066    &0.00076    &0.00071    \\
&   L20ALM     &0.x    &0.1564    &0.2549    &0.2461    &0.2439    &0.2447    &0.3701    &0.3801    &0.4002    &0.4208\\%巨慢
&   Our\_L1             &0.x    &0.3219    &0.3655    &0.4058    &0.4239    &0.4609    &0.4772    &0.4933    &0.4993    &0.5326 \\
&   Our\_L1\_center      &0.x    &0.3219    &0.3832    &0.4031    &0.4328    &0.4735    &0.5105    &0.5253    &0.5294    &0.5571 \\
&   Our        &0.x    &0.x    &0.4093    &0.4560    &0.4692    &0.5104    &0.5320    &0.5689    &0.5823    &0.5918 \\
&   Our\_nor\_con    &0.x    &0.2715    &0.3088    &0.3759    &0.4039    &0.4459    &0.4597    &0.5108    &0.5627    &0.5793   \\
&   center\_semantic   &0.x    &0.2791    &0.3117    &0.3665    &0.3688    &0.4159    &0.4277    &0.4546    &0.4864    &0.4933 \\
&   center\_binary      &0.x    &0.1546    &0.1845    &0.2470    &0.2883    &0.2788    &0.3693    &0.3663    &0.4026    &0.4094 \\
&   Our\_L1\_s\_binary       &0.x    &0.3178    &0.3499    &0.4354    &0.4158    &0.4605    &0.4578    &0.4667    &0.4772    &0.4840 \\
&   LASSO0.1        &0.x    &0.1546    &0.1845    &0.2470    &0.2883    &0.2788    &0.3693    &0.3663    &0.4026    &0.4094    \\
&   Our\_L1\_center\_b        &0.x    &0.3178    &0.3499    &0.4354    &0.4158    &0.4605    &0.4578    &0.4685    &0.4772    &0.4840    \\
\hline
\end{tabular}
\label{tab_ndcg_results}
\end{table*}

==> result_clustering.tex <==
\begin{table*}[htb]
\caption{Clustering results on SUN dataset.}
\centering % used for centering table
\begin{tabular}{l|l|rrrrrrrrrr}
\hline
    &Method & 5 & 10 & 15 & 20 & 25 &30 &35 &40 &45 &50  \\
\hline
\multirow{7}{*}{ACC} &
    Random          &0.2416    &0.2729    &0.2921    &0.3062    &0.3220    &0.3379    &0.3503    &0.3607    &0.3703    &0.3802 \\
%&   LapScore      &0.2300    &0.2350    &0.3600    &0.4650    &0.4750    &0.4600    &0.4800    &0.5150    &0.5450    &0.4700  \\
&   MCFS          &0.2500    &0.3150    &0.3750    &0.3850    &0.4300    &0.3850    &0.3900    &0.4200    &0.4850    &0.5050 \\
&   TRACK         &0.1400    &0.1950    &0.2450    &0.2300    &0.2300    &0.2350    &0.2450    &0.2900    &0.2900    &0.2450 \\
&   FSASL15       &0.2421    &0.3052    &0.3715    &0.3930    &0.3948    &0.4241    &0.4395    &0.4405    &0.4841    &0.4544 \\ %alpha=1
%&   LASSO        &0.2400    &0.3100    &0.4550    &0.4500    &0.4850    &0.4950    &0.4850    &0.4850    &0.4400    &0.4900 \\ %lasso
&   LASSO\_con1        &0.3200    &0.3300    &0.3600    &0.4000    &0.4300    &0.4500    &0.4700    &0.4850    &0.4900    &0.4900 \\ %lasso_con
&   L20ALM     &0.2450    &0.2850    &0.2800    &0.3400    &0.3000    &0.3050    &0.3850    &0.3900    &0.4300    &0.4050\\%巨慢
&   Our\_L1             &0.3250    &0.4050    &0.4500    &0.5050    &0.5450    &0.4500    &0.5950    &0.5700    &0.4650    &0.6150 \\
&   Our\_L1\_center      &0.3800    &0.4500    &0.4450    &0.5000    &0.5300    &0.5200    &0.5500    &0.5800    &0.5950    &0.6200 \\
&   Our\_L1\_center\_b      &0.2900    &0.3950    &0.3500    &0.5000    &0.4750    &0.5050    &0.5350    &0.4400    &0.5350    &0.5850 \\
&   Our         &0.1900    &0.3000    &0.2700    &0.3050    &0.2750    &0.3900    &0.3550    &0.3450    &0.3600    &0.4400  \\%lasso
&   Our\_con         &0.1700    &0.2150    &0.2400    &0.3400    &0.3000    &0.3400    &0.3600    &0.3750    &0.4450    &0.4400 \\ %lasso_con
&   Our\_nor    &0.3550    &0.3850    &0.4100    &0.4150    &0.4400    &0.5500    &0.4950    &0.5000    &0.5400    &0.5600   \\ %lasso
&   Our\_nor\_con0.1    &0.2300    &0.3750    &0.4100    &0.4700    &0.4000    &0.4850    &0.4750    &0.4750    &0.5200    &0.5650   \\ %lasso_con
&   Our\_nor\_con1    &0.3900    &0.3900    &0.4350    &0.3950    &0.4900    &0.5250    &0.5500    &0.5650    &0.6100    &0.5850   \\ %lasso_con
&   Our\_remove\_red  &0.3400    &0.3750    &0.4400    &0.4850    &0.5800    &0.5450    &0.5250    &0.5550    &0.5450    &0.5200 \\
&   Our\_snor    &0.2450    &0.2550    &0.2750    &0.3100    &0.3850    &0.4450    &0.4400    &0.4900    &0.4500    &0.5200   \\ %lasso
&   Our\_snor\_con    &0.2000    &0.2500    &0.2700    &0.2950    &0.3900    &0.3750    &0.3700    &0.3850    &0.5050    &0.5100   \\ %lasso_con
&   Our\_nor\_con\_R    &0.2300    &0.3750    &0.4100    &0.4700    &0.4000    &0.4850    &0.4750    &0.4725    &0.5250    &0.5225 \\
&   center\_semantic          &0.3000    &0.3200    &0.3500    &0.4650    &0.4950    &0.4900    &0.5450    &0.5350    &0.5800    &0.5850 \\
&   center\_binary      &0.1800    &0.2150    &0.2300    &0.2800    &0.2750    &0.3900    &0.3900    &0.3600    &0.3850    &0.4600 \\
&   LASSO\_con0.1        &0.1800    &0.2250    &0.2200    &0.2950    &0.3350    &0.3050    &0.4000    &0.3800    &0.3950    &0.4400 \\ %lasso_con
\hline
\multirow{7}{*}{NMI} &
    Random          &0.1803    &0.2188    &0.2398    &0.2552    &0.2721    &0.2887    &0.3054    &0.3170    &0.3296    &0.3393 \\
%&   LapScore      &0.2492    &0.2985    &0.3911    &0.4829    &0.4492    &0.4651    &0.4864    &0.5036    &0.5103    &0.5086  \\
&   MCFS          &0.2166    &0.2537    &0.3285    &0.3449    &0.3905    &0.3790    &0.4144    &0.4360    &0.4508    &0.4723 \\
&   TRACK         &0.0872    &0.1323    &0.2150    &0.1986    &0.1895    &0.2046    &0.1942    &0.2176    &0.2181    &0.1939 \\
&   FSASL15        &0.1246    &0.1718    &0.2207    &0.2743    &0.2827    &0.3208    &0.3362    &0.3470    &0.3680    &0.3697 \\
%&   LASSO        &0.2069    &0.3127    &0.3859    &0.3732    &0.4137    &0.4486    &0.4249    &0.4228    &0.4105    &0.4381    \\%lasso
&   LASSO\_con1        &0.2996    &0.3396    &0.3567    &0.3861    &0.4174    &0.4364    &0.4510    &0.4789    &0.4803    &0.4874 \\ %lasso_con
&   L20ALM     &0.2005    &0.2356    &0.2630    &0.3206    &0.2584    &0.2493    &0.3259    &0.3172    &0.3952    &0.3512\\%巨慢
&   Our\_L1             &0.3099    &0.4086    &0.4181    &0.4735    &0.4763    &0.4511    &0.5404    &0.5267    &0.5158    &0.5400 \\
&   Our\_L1\_center      &0.3504    &0.4057    &0.4274    &0.4614    &0.4929    &0.4771    &0.5085    &0.5375    &0.5240    &0.5417 \\
&   Our\_L1\_center\_b      &0.2915    &0.3811    &0.3541    &0.4418    &0.4304    &0.4786    &0.5129    &0.4459    &0.5341    &0.5032 \\
&   Our        &0.2143    &0.3259    &0.3109    &0.3454    &0.3421    &0.3943    &0.3937    &0.3748    &0.3894    &0.4091 \\ %lasso
&   Our\_con        &0.1568    &0.2261    &0.2348    &0.3035    &0.3238    &0.3886    &0.3476    &0.3699    &0.4285    &0.4352 \\ %lasso_con
&   Our\_nor   &0.3274    &0.3689    &0.3931    &0.3971    &0.4006    &0.4756    &0.4915    &0.4811    &0.5345    &0.5023 \\ %lasso
&   Our\_nor\_con0.1   &0.2287    &0.3231    &0.3668    &0.4234    &0.4210    &0.4591    &0.4621    &0.4632    &0.4881    &0.5335 \\  %lasso_con
&   Our\_nor\_con1    &0.3533    &0.3873    &0.4313    &0.4022    &0.4786    &0.4828    &0.4944    &0.5132    &0.5385    &0.5144   \\ %lasso_con
&   Our\_remove\_red &0.3334    &0.3705    &0.4016    &0.4099    &0.5211    &0.4925    &0.4873    &0.5225    &0.4967    &0.5024 \\
&   Our\_snor    &0.2592    &0.2748    &0.3133    &0.3391    &0.3714    &0.4087    &0.4295    &0.4473    &0.4344    &0.4593   \\ %lasso
&   Our\_snor\_con    &0.1513    &0.2337    &0.2963    &0.3268    &0.3378    &0.3819    &0.3927    &0.3785    &0.4837    &0.4899   \\ %lasso_con
&   Our\_nor\_con\_R    &0.2287    &0.3231    &0.3668    &0.4234    &0.4210    &0.4591    &0.4621    &0.4523    &0.4841    &0.4977 \\
&   center\_semantic          &0.2948    &0.3329    &0.3662    &0.4587    &0.4782    &0.4576    &0.5250    &0.5361    &0.5415    &0.5721 \\
&   center\_binary      &0.0997    &0.1671    &0.1914    &0.2606    &0.2608    &0.3264    &0.3518    &0.3675    &0.3544    &0.4264 \\
&   LASSO\_con0.1        &0.0997    &0.1950    &0.1801    &0.2706    &0.3125    &0.3075    &0.3343    &0.3860    &0.4234    &0.4363    \\%lasso_con
\hline
\end{tabular}
\label{tab_ndcg_results}
\end{table*}

\begin{table*}[htb]
\caption{Clustering results on SUN10 dataset.}
\centering % used for centering table
\begin{tabular}{l|l|rrrrrrrrrr}
\hline
    &Method & 10 & 20 & 30 & 40 & 50 &60 &70 &80 &90 &100  \\
\hline
\multirow{7}{*}{ACC} &
    Random          &0.2739    &0.3044    &0.3331    &0.3469    &0.3745    &0.3935    &0.4037    &0.4320    &0.4409    &0.4502 \\
&   LapScore      &0.x    &0.2350    &0.3600    &0.4650    &0.4750    &0.4600    &0.4800    &0.5150    &0.5450    &0.4700  \\
&   MCFS          &0.x    &0.3150    &0.3750    &0.3850    &0.4300    &0.3850    &0.3900    &0.4200    &0.4850    &0.5050 \\
&   FSASL15       &0.x    &0.3052    &0.3715    &0.3930    &0.3948    &0.4241    &0.4395    &0.4405    &0.4841    &0.4544 \\ %alpha=1
%&   LASSO        &0.x    &0.3100    &0.4550    &0.4500    &0.4850    &0.4950    &0.4850    &0.4850    &0.4400    &0.4900 \\ %lasso
&   LASSO\_con        &0.2150    &0.2800    &0.3900    &0.3600    &0.4600    &0.4350    &0.4550    &0.4900    &0.4350    &0.4650 \\ %lasso_con
&   L20ALM     &0.x    &0.x    &0.2113    &0.2331    &0.2405    &0.2614    &0.2771    &0.2743    &0.2916    &0.3081\\%巨慢
%&   Our         &0.x    &0.3000    &0.2700    &0.3050    &0.2750    &0.3900    &0.3550    &0.3450    &0.3600    &0.4400  \\%lasso
&   Our\_con         &0.2150    &0.3400    &0.3400    &0.3750    &0.4400    &0.3850    &0.4350    &0.4425    &0.4750    &0.4100 \\ %lasso_con
%&   Our\_nor    &0.x    &0.3850    &0.4100    &0.4150    &0.4400    &0.5500    &0.4950    &0.5000    &0.5400    &0.5600   \\ %lasso
&   Our\_nor\_con    &0.3750    &0.4700    &0.4850    &0.4750    &0.5650    &0.6000    &0.6250    &0.5950    &0.6000    &0.5450   \\ %lasso_con
%&   Our\_snor    &0.x    &0.2550    &0.2750    &0.3100    &0.3850    &0.4450    &0.4400    &0.4900    &0.4500    &0.5200   \\ %lasso
&   Our\_snor\_con    &0.2500    &0.2950    &0.3750    &0.3850    &0.5100    &0.4700    &0.4800    &0.5400    &0.4600    &0.4800   \\ %lasso_con
\hline
\multirow{7}{*}{NMI} &
    Random          &0.2141    &0.2532    &0.2842    &0.3061    &0.3307    &0.3592    &0.3720    &0.3974    &0.4078    &0.4246 \\
&   LapScore      &0.x    &0.2985    &0.3911    &0.4829    &0.4492    &0.4651    &0.4864    &0.5036    &0.5103    &0.5086  \\
&   MCFS          &0.x    &0.2537    &0.3285    &0.3449    &0.3905    &0.3790    &0.4144    &0.4360    &0.4508    &0.4723 \\
&   FSASL15        &0.x    &0.1718    &0.2207    &0.2743    &0.2827    &0.3208    &0.3362    &0.3470    &0.3680    &0.3697 \\
%&   LASSO        &0.x    &0.3127    &0.3859    &0.3732    &0.4137    &0.4486    &0.4249    &0.4228    &0.4105    &0.4381    \\%lasso
&   LASSO\_con        &0.1671    &0.2606    &0.3264    &0.3675    &0.4264    &0.4483    &0.4568    &0.4958    &0.5000    &0.4882    \\%lasso_con
&   L20ALM     &0.x    &0.1452    &0.2113    &0.2331    &0.2405    &0.2614    &0.2771    &0.2743    &0.2916    &0.3081\\%巨慢
%&   Our        &0.x    &0.3259    &0.3109    &0.3454    &0.3421    &0.3943    &0.3937    &0.3748    &0.3894    &0.4091 \\ %lasso
&   Our\_con        &0.2261    &0.3035    &0.3886    &0.3699    &0.4352    &0.4031    &0.4033    &0.4505    &0.4619    &0.4206 \\ %lasso_con
%&   Our\_nor   &0.x    &0.3689    &0.3931    &0.3971    &0.4006    &0.4756    &0.4915    &0.4811    &0.5345    &0.5023 \\ %lasso
&   Our\_nor\_con   &0.3231    &0.4234    &0.4591    &0.4632    &0.5335    &0.5505    &0.5966    &0.5622    &0.5671    &0.5543 \\  %lasso_con
%&   Our\_snor    &0.x    &0.2748    &0.3133    &0.3391    &0.3714    &0.4087    &0.4295    &0.4473    &0.4344    &0.4593   \\ %lasso
&   Our\_snor\_con    &0.2337    &0.3268    &0.3819    &0.3785    &0.4899    &0.4369    &0.4481    &0.5457    &0.4852    &0.4864   \\ %lasso_con
\hline
\end{tabular}
\label{tab_ndcg_results}
\end{table*}


\begin{table*}[htb]
\caption{Clustering results on AwA\_my\_deep dataset.}
\centering % used for centering table
\begin{tabular}{l|l|rrrrrrrrrr}
\hline
    &Method & 5 & 10 & 15 & 20 & 25 &30 &35 &40 &45 &50  \\
\hline
\multirow{7}{*}{ACC} &
    Random          &0.2023    &0.2247    &0.2376    &0.2508    &0.2627    &0.2750    &0.2859    &0.2960    &0.3087    &0.3189 \\
%&   LapScore      &x    &0.2150    &0.2100    &0.2100    &0.2050    &0.2450    &0.2800    &0.2800    &0.2950    &0.2750  \\
&   MCFS          &0.2340    &0.2901    &0.3230    &0.3388    &0.3430    &0.3604    &0.3550    &0.3722    &0.3788    &0.3898 \\
&   TRACK         &0.2484    &0.2785    &0.3165    &0.3654    &0.3837    &0.3994    &0.3981    &0.3642    &0.3693    &0.4215 \\
&   FSASL15       &0.2408    &0.3032    &0.3660    &0.3746    &0.4006    &0.4199    &0.4291    &0.4228    &0.4529    &0.4537 \\ %alpha=1
&   LASSO        &0.2023    &0.2673    &0.3186    &0.3254    &0.3451    &0.3592    &0.3584    &0.3608    &0.3788    &0.3921    \\
&   L20ALM     &0.2367    &0.2840    &0.3183    &0.4023    &0.3926    &0.3739    &0.4126    &0.4163    &0.4353    &0.4405\\%巨慢
&   Our        &0.2160    &0.2492    &0.2828    &0.3018    &0.2971    &0.3131    &0.2793    &0.3139    &0.3227    &0.3243 \\
&   Our\_nor\_con    &0.2574    &0.2851    &0.2939    &0.3506    &0.3495    &0.3639    &0.3754    &0.4348    &0.4411    &0.4565   \\ %lasso_con
&   Our\_snor\_con    &0.2610    &0.2845    &0.2720    &0.3071    &0.3184    &0.3722    &0.3595    &0.3799    &0.3862    &0.3730   \\ %lasso_con
&   Our\_nor\_con\_R    &0.2574    &0.2851    &0.3015    &0.3467    &0.3495    &0.3621    &0.3754    &0.4348    &0.4411    &0.4265 \\
&   center\_semantic    &0.1995    &0.2780    &0.2982    &0.3547    &0.3892    &0.4332    &0.4685    &0.4655    &0.4992    &0.4972 \\
&   center\_binary      &0.2023    &0.2673    &0.3186    &0.3254    &0.3451    &0.3592    &0.3584    &0.3608    &0.3788    &0.3921 \\
&   Our\_center\_L1      &0.2454    &0.3087    &0.3751    &0.3704    &0.4006    &0.4367    &0.4424    &0.4405    &0.4416    &0.4587 \\
\hline
\multirow{7}{*}{NMI} &
    Random          &0.0725    &0.0997    &0.1122    &0.1288    &0.1432    &0.1540    &0.1691    &0.1834    &0.1948    &0.2078 \\
%&   LapScore      &0.x    &0.1822    &0.2004    &0.2104    &0.2021    &0.2613    &0.2842    &0.2842    &0.2930    &0.2946  \\
&   MCFS          &0.1363    &0.1947    &0.2253    &0.2321    &0.2284    &0.2651    &0.2811    &0.2756    &0.2876    &0.2994 \\
&   TRACK         &0.1476    &0.1781    &0.2191    &0.2464    &0.2738    &0.2873    &0.2930    &0.2990    &0.3014    &0.3221 \\
&   FSASL15       &0.1205    &0.1668    &0.2187    &0.2758    &0.2869    &0.3121    &0.3323    &0.3360    &0.3637    &0.3729 \\ %alpha=1
&   LASSO        &0.0932    &0.1698    &0.1977    &0.2113    &0.2248    &0.2285    &0.2321    &0.2362    &0.2603    &0.2738    \\
&   L20ALM     &0.1440    &0.1910    &0.2130    &0.2634    &0.2830    &0.2659    &0.2978    &0.3240    &0.3474    &0.3461\\%巨慢
&   Our        &0.1224    &0.1623    &0.1824    &0.1832    &0.1989    &0.2091    &0.2088    &0.2119    &0.2334    &0.2472 \\
&   Our\_nor\_con    &0.1703    &0.1970    &0.2201    &0.2763    &0.2879    &0.2991    &0.3109    &0.3402    &0.3534    &0.3611   \\ %lasso_con
&   Our\_snor\_con    &0.1879    &0.1883    &0.1953    &0.2080    &0.2279    &0.2639    &0.2745    &0.2743    &0.2808    &0.2780   \\ %lasso_con
&   Our\_nor\_con\_R    &0.1703    &0.1970    &0.2250    &0.2769    &0.2879    &0.2982    &0.3109    &0.3402    &0.3534    &0.3611 \\
&   center\_semantic   &0.0953    &0.1525    &0.1683    &0.2504    &0.2614    &0.3225    &0.3562    &0.3611    &0.4029    &0.4049 \\
&   center\_binary     &0.0932    &0.1698    &0.1977    &0.2113    &0.2248    &0.2285    &0.2321    &0.2362    &0.2603    &0.2738\\
&   Our\_center\_L1    &0.1724    &0.2014    &0.2563    &0.3118    &0.3320    &0.3369    &0.3556    &0.3631    &0.3682    &0.3785 \\
\hline
\end{tabular}
\label{tab_ndcg_results}
\end{table*}

\begin{table*}[htb]
\caption{Clustering results on AwA\_Guo\_deep dataset.}
\centering % used for centering table
\begin{tabular}{l|l|rrrrrrrrrr}
\hline
    &Method & 5 & 10 & 15 & 20 & 25 &30 &35 &40 &45 &50  \\
\hline
\multirow{7}{*}{ACC} &
    Random          &0.2248    &0.2639    &0.2950    &0.3088    &0.3253    &0.3359    &0.3558    &0.3740    &0.3985    &0.4194 \\
%&   LapScore      &x    &0.2150    &0.2100    &0.2100    &0.2050    &0.2450    &0.2800    &0.2800    &0.2950    &0.2750  \\
&   MCFS          &0.x    &0.2901    &0.3230    &0.3388    &0.3430    &0.3604    &0.3550    &0.3722    &0.3788    &0.3898 \\
&   FSASL15       &0.2689    &0.3294    &0.3657    &0.3748    &0.4893    &0.5401    &0.5479    &0.5893    &0.6000    &0.6065 \\ %alpha=1
&   LASSO        &0.x    &0.2673    &0.3186    &0.3254    &0.3451    &0.3592    &0.3584    &0.3608    &0.3788    &0.3921    \\
&   L20ALM     &0.2641    &0.3134    &0.3587    &0.4561    &0.4639    &0.4969    &0.5322    &0.5426    &0.5354    &0.5549\\%巨慢
&   Our        &0.x    &0.2492    &0.2828    &0.3018    &0.2971    &0.3131    &0.2793    &0.3139    &0.3227    &0.3243 \\
&   Our\_nor\_con    &0.2943    &0.3867    &0.4165    &0.4398    &0.4350    &0.4793    &0.4828    &0.5173    &0.5188    &0.5636   \\ %lasso_con
&   Our\_snor\_con    &0.x    &0.2845    &0.2720    &0.3071    &0.3184    &0.3722    &0.3595    &0.3799    &0.3862    &0.3730   \\ %lasso_con
\hline
\multirow{7}{*}{NMI} &
    Random          &0.1071    &0.1555    &0.1809    &0.2020    &0.2216    &0.2402    &0.2554    &0.2814    &0.3044    &0.3259 \\
%&   LapScore      &0.x    &0.1822    &0.2004    &0.2104    &0.2021    &0.2613    &0.2842    &0.2842    &0.2930    &0.2946  \\
&   MCFS          &0.x    &0.1947    &0.2253    &0.2321    &0.2284    &0.2651    &0.2811    &0.2756    &0.2876    &0.2994 \\
&   FSASL15       &0.1416    &0.1977    &0.2631    &0.2894	&0.3591    &0.4155    &0.4551    &0.4965		&0.5131    &0.5261 \\ %alpha=1
&   LASSO        &0.x    &0.1698    &0.1977    &0.2113    &0.2248    &0.2285    &0.2321    &0.2362    &0.2603    &0.2738    \\
&   L20ALM     &0.1981    &0.2259    &0.2455    &0.3573    &0.3837    &0.4129    &0.4703    &0.4744    &0.4900    &0.5133\\%巨慢
&   Our        &0.x    &0.1623    &0.1824    &0.1832    &0.1989    &0.2091    &0.2088    &0.2119    &0.2334    &0.2472 \\
&   Our\_nor\_con    &0.2589    &0.3316    &0.3491    &0.3596    &0.3756    &0.4199    &0.4277    &0.4587    &0.4673    &0.5045   \\ %lasso_con
&   Our\_snor\_con    &0.x    &0.1883    &0.1953    &0.2080    &0.2279    &0.2639    &0.2745    &0.2743    &0.2808    &0.2780   \\ %lasso_con
\hline
\end{tabular}
\label{tab_ndcg_results}
\end{table*}

\begin{table*}[htb]
\caption{Clustering results on AwA\_SIFT dataset.}
\centering % used for centering table
\begin{tabular}{l|l|rrrrrrrrrr}
\hline
    &Method & 5 & 10 & 15 & 20 & 25 &30 &35 &40 &45 &50  \\
\hline
\multirow{7}{*}{ACC} &
    Random          &0.1997    &0.2128    &0.2209    &0.2280    &0.2325    &0.2337    &0.2341    &0.2360    &0.2364    &0.2372 \\
%&   LapScore      &x    &0.2150    &0.2100    &0.2100    &0.2050    &0.2450    &0.2800    &0.2800    &0.2950    &0.2750  \\
&   MCFS          &0.x    &0.2901    &0.3230    &0.3388    &0.3430    &0.3604    &0.3550    &0.3722    &0.3788    &0.3898 \\
&   FSASL15       &0.x    &0.3032    &0.3660    &0.3746    &0.4006    &0.4199    &0.4291    &0.4228    &0.4529    &0.4537 \\ %alpha=1
&   LASSO        &0.1981    &0.2178    &0.2464    &0.2549    &0.2455    &0.2604    &0.2668    &0.2762    &0.2503    &0.2608    \\
&   L20ALM     &0.2294    &0.2121    &0.2447    &0.2456    &0.2516    &0.2388    &0.2451    &0.2463    &0.2312    &0.2608\\%巨慢
&   Our        &0.x    &0.2492    &0.2828    &0.3018    &0.2971    &0.3131    &0.2793    &0.3139    &0.3227    &0.3243 \\
&   Our\_nor\_con    &0.2028    &0.2437    &0.2307    &0.2432    &0.2464    &0.2560    &0.2450    &0.2531    &0.2439    &0.2526   \\ %lasso_con
&   Our\_snor\_con    &0.x    &0.2845    &0.2720    &0.3071    &0.3184    &0.3722    &0.3595    &0.3799    &0.3862    &0.3730   \\ %lasso_con
\hline
\multirow{7}{*}{NMI} &
    Random          &0.0696    &0.0808    &0.0907    &0.0956    &0.1001    &0.1023    &0.1056    &0.1063    &0.1068    &0.1089 \\
%&   LapScore      &0.x    &0.1822    &0.2004    &0.2104    &0.2021    &0.2613    &0.2842    &0.2842    &0.2930    &0.2946  \\
&   MCFS          &0.x    &0.1947    &0.2253    &0.2321    &0.2284    &0.2651    &0.2811    &0.2756    &0.2876    &0.2994 \\
&   FSASL15       &0.x    &0.1668    &0.2187    &0.2758    &0.2869    &0.3121    &0.3323    &0.3360    &0.3637    &0.3729 \\ %alpha=1
&   LASSO        &0.0677    &0.0903    &0.1101    &0.1154    &0.1245    &0.1296    &0.1377    &0.1385    &0.1306    &0.1356    \\
&   L20ALM     &0.1099    &0.1147    &0.1095    &0.1010    &0.1025    &0.1160    &0.1173    &0.1267    &0.1059    &0.1332\\%巨慢
&   Our        &0.x    &0.1623    &0.1824    &0.1832    &0.1989    &0.2091    &0.2088    &0.2119    &0.2334    &0.2472 \\
&   Our\_nor\_con    &0.0697    &0.1260    &0.1312    &0.1300    &0.1375    &0.1411    &0.1404    &0.1372    &0.1339    &0.1303   \\ %lasso_con
&   Our\_snor\_con    &0.x    &0.1883    &0.1953    &0.2080    &0.2279    &0.2639    &0.2745    &0.2743    &0.2808    &0.2780   \\ %lasso_con
\hline
\end{tabular}
\label{tab_ndcg_results}
\end{table*}


\begin{table*}[htb]
\caption{Clustering results on aPY\_deep dataset.}
\centering % used for centering table
\begin{tabular}{l|l|rrrrrrrrrr}
\hline
    &Method & 5 & 10 & 15 & 20 & 25 &30 &35 &40 &45 &50  \\
\hline
\multirow{7}{*}{ACC} &
    Random          &0.2201    &0.2721    &0.2924    &0.3196    &0.3387    &0.3668    &0.3814    &0.4055    &0.4283    &0.4348 \\
%&   LapScore      &x    &0.2150    &0.2100    &0.2100    &0.2050    &0.2450    &0.2800    &0.2800    &0.2950    &0.2750  \\
&   MCFS          &0.2315    &0.2961    &0.3045    &0.3249    &0.3517    &0.3850    &0.4009    &0.4486    &0.4523    &0.4637 \\
&   FSASL15       &0.2008    &0.2424    &0.2924    &0.3234    &0.3483    &0.3763    &0.3941    &0.3926    &0.4115    &0.4535 \\ %alpha=1
&   LASSO1        &0.2863    &0.3028    &0.3464    &0.3718    &0.4097    &0.4240    &0.4618    &0.4918    &0.5237    &0.5285 \\
&   L20ALM     &0.2068    &0.2356    &0.3132    &0.3302    &0.3483    &0.3336    &0.4459    &0.4179    &0.4266    &0.4705\\%巨慢
&   Our\_L1             &0.2943    &0.3343    &0.4051    &0.4266    &0.4792    &0.5064    &0.5397    &0.5216    &0.5333    &0.5719 \\
&   Our\_L1\_center      &0.2943    &0.3343    &0.4138    &0.4372    &0.4663    &0.5310    &0.5915    &0.5484    &0.5711    &0.5919 \\
&   Our        &0.2992    &0.3604    &0.4826    &0.5023    &0.5064    &0.5450    &0.5261    &0.5753    &0.5828    &0.5930 \\
&   Our\_nor\_con    &0.2697    &0.2995    &0.3563    &0.3918    &0.4459    &0.4750    &0.4773    &0.5378    &0.6097    &0.5934   \\ %lasso_con
%&   Our\_snor\_con    &0.3113    &0.3290    &0.4020    &0.4576    &0.5148    &0.5136    &0.5234    &0.6010    &0.6023    &0.6547   \\ %lasso_con
%&   Our\_nor\_con\_R    &0.2697    &0.2995    &0.3563    &0.3918    &0.4459    &0.4750    &0.4773    &0.5378    &0.6097    &0.5934   \\
&   center\_semantic   &0.2254    &0.3014    &0.3737    &0.4257    &0.4007    &0.4357    &0.4650    &0.4766    &0.4879    &0.5034 \\
&   center\_binary      &0.2144    &0.2470    &0.2765    &0.3056    &0.3498    &0.3238    &0.3952    &0.3865    &0.4115    &0.4138 \\
&   Our\_L1\_s\_binary       &0.2421    &0.3487    &0.3336    &0.4603    &0.4576    &0.4864    &0.4868    &0.4902    &0.5291    &0.5238 \\
&   LASSO0.1        &0.2144    &0.2470    &0.2765    &0.3056    &0.3498    &0.3238    &0.3952    &0.3865    &0.4115    &0.4138    \\
&   Our\_L1\_center\_b        &0.2421    &0.3487    &0.3336    &0.4603    &0.4576    &0.4864    &0.4868    &0.5008    &0.5291    &0.5238    \\
\hline
\multirow{7}{*}{NMI} &
    Random          &0.1381    &0.1999    &0.2242    &0.2535    &0.2767    &0.3029    &0.3246    &0.3439    &0.3649    &0.3833 \\
%&   LapScore      &0.x    &0.1822    &0.2004    &0.2104    &0.2021    &0.2613    &0.2842    &0.2842    &0.2930    &0.2946  \\
&   MCFS          &0.1839    &0.2780    &0.2881    &0.2899    &0.3428    &0.3800    &0.4062    &0.4309    &0.4399    &0.4550 \\
&   FSASL15        &0.1165    &0.1420    &0.2124    &0.2431    &0.2746    &0.2921    &0.3275    &0.3230    &0.3494    &0.3893 \\
&   LASSO1        &0.2380    &0.2954    &0.3022    &0.3453    &0.3809    &0.4167    &0.4261    &0.4826    &0.4936    &0.5023    \\
&   L20ALM     &0.1172    &0.1564    &0.2549    &0.2461    &0.2439    &0.2447    &0.3701    &0.3801    &0.4002    &0.4208\\%巨慢
&   Our\_L1             &0.2815    &0.3219    &0.3655    &0.4058    &0.4239    &0.4609    &0.4772    &0.4933    &0.4993    &0.5326 \\
&   Our\_L1\_center      &0.2815    &0.3219    &0.3832    &0.4031    &0.4328    &0.4735    &0.5105    &0.5253    &0.5294    &0.5571 \\
&   Our        &0.2354    &0.2921    &0.4093    &0.4560    &0.4692    &0.5104    &0.5320    &0.5689    &0.5823    &0.5918 \\
&   Our\_nor\_con    &0.2518    &0.2715    &0.3088    &0.3759    &0.4039    &0.4459    &0.4597    &0.5108    &0.5627    &0.5793   \\ %lasso_con
%&   Our\_snor\_con    &0.2514    &0.3072    &0.3840    &0.4537    &0.5149    &0.5341    &0.5534    &0.5970    &0.6202    &0.6513   \\ %lasso_con
%&   Our\_nor\_con\_R    &0.2518    &0.2715    &0.3088    &0.3759    &0.4039    &0.4459    &0.4597    &0.5108    &0.5627    &0.5793   \\
&   center\_semantic   &0.1566    &0.2791    &0.3117    &0.3665    &0.3688    &0.4159    &0.4277    &0.4546    &0.4864    &0.4933 \\
&   center\_binary      &0.1312    &0.1546    &0.1845    &0.2470    &0.2883    &0.2788    &0.3693    &0.3663    &0.4026    &0.4094 \\
&   Our\_L1\_s\_binary       &0.2079    &0.3178    &0.3499    &0.4354    &0.4158    &0.4605    &0.4578    &0.4667    &0.4772    &0.4840 \\
&   LASSO0.1        &0.1312    &0.1546    &0.1845    &0.2470    &0.2883    &0.2788    &0.3693    &0.3663    &0.4026    &0.4094    \\
&   Our\_L1\_center\_b        &0.2079    &0.3178    &0.3499    &0.4354    &0.4158    &0.4605    &0.4578    &0.4685    &0.4772    &0.4840    \\
\hline
\end{tabular}
\label{tab_ndcg_results}
\end{table*}

\begin{table*}[htb]
\caption{Clustering results on CIFAR10\_2\_8 dataset.}
\centering % used for centering table
\begin{tabular}{l|l|rrrrrrrrrr}
\hline
    &Method & 5 & 10 & 15 & 20 & 25 &30 &35 &40 &45 &50  \\
\hline
\multirow{7}{*}{ACC} &
    Random          &0.1688    &0.1868    &0.2048    &0.2113    &0.2198    &0.2274    &0.2355    &0.2413    &0.2519    &0.2473 \\
&   MCFS          &0.2034    &0.1887    &0.2031    &0.2068    &0.2445    &0.2262    &0.2513    &0.2501    &0.2847    &0.2433 \\
&   FSASL15       &0.1756    &0.1636    &0.1689    &0.1922    &0.1937    &0.2000    &0.2195    &0.2476    &0.2569    &0.2581 \\ %alpha=1
&   LASSO1        &0.2079    &0.2309    &0.3039    &0.2828    &0.2889    &0.3321    &0.3524    &0.3289    &0.2953    &0.2951 \\
&   L20ALM     &0.2016    &0.2365    &0.3145    &0.2731    &0.3309    &0.2741    &0.3012    &0.2853    &0.3359    &0.3500\\%巨慢
&   Our\_L1             &0.2660    &0.2820    &0.3161    &0.3497    &0.3448    &0.2910    &0.3580    &0.3410    &0.3471    &0.3502 \\
&   Our\_L1\_center      &0.2660    &0.2820    &0.3021    &0.3410    &0.3519    &0.3673    &0.3797    &0.3627    &0.3679    &0.3722 \\
&   Our        &0.2578    &0.3148    &0.2768    &0.3023    &0.3224    &0.3974    &0.3741    &0.3297    &0.3304    &0.3539 \\
&   Our\_L1\_s\_binary       &0.x    &0.3487    &0.3336    &0.4603    &0.4576    &0.4864    &0.4868    &0.4902    &0.5291    &0.5238 \\
&   Our\_L1\_center\_b        &0.x    &0.3487    &0.3336    &0.4603    &0.4576    &0.4864    &0.4868    &0.5008    &0.5291    &0.5238    \\
\hline
\multirow{7}{*}{NMI} &
    Random          &0.0368    &0.0455    &0.0610    &0.0620    &0.0683    &0.0766    &0.0888    &0.0887    &0.0963    &0.0965 \\
&   MCFS          &0.0604    &0.0386    &0.0692    &0.0953    &0.1129    &0.1005    &0.1198    &0.1023    &0.1248    &0.0962 \\
&   FSASL15        &0.0346    &0.0293    &0.0401    &0.0449    &0.0403    &0.0514    &0.0638    &0.0930    &0.0941    &0.1047 \\
&   LASSO1        &0.0563    &0.0842    &0.1556    &0.1353    &0.1084    &0.1688    &0.1987    &0.1733    &0.1311    &0.1382    \\
&   L20ALM     &0.0638    &0.0765    &0.1236    &0.1394    &0.1665    &0.1269    &0.1480    &0.1377    &0.1541    &0.1980\\%巨慢
&   Our\_L1             &0.1066    &0.1097    &0.1540    &0.1698    &0.1935    &0.1416    &0.1911    &0.1953    &0.2050    &0.2072 \\
&   Our\_L1\_center      &0.1166    &0.1107    &0.1396    &0.1798    &0.1822    &0.1814    &0.1972    &0.2009    &0.2089    &0.2117 \\
&   Our        &0.1022    &0.1338    &0.1192    &0.1499    &0.1726    &0.2080    &0.1832    &0.1393    &0.1880    &0.2047 \\
&   Our\_L1\_s\_binary       &0.x    &0.3178    &0.3499    &0.4354    &0.4158    &0.4605    &0.4578    &0.4667    &0.4772    &0.4840 \\
&   Our\_L1\_center\_b        &0.x    &0.3178    &0.3499    &0.4354    &0.4158    &0.4605    &0.4578    &0.4685    &0.4772    &0.4840    \\
\hline
\end{tabular}
\label{tab_ndcg_results}
\end{table*}

%\begin{table*}[htb]
%\caption{Clustering results on CIFAR10 dataset.}
%\centering % used for centering table
%\begin{tabular}{l|l|rrrrrrrrrr}
%\hline
%    &Method & 5 & 10 & 15 & 20 & 25 &30 &35 &40 &45 &50  \\
%\hline
%\multirow{7}{*}{ACC} &
%    Random          &0.3325    &0.3644    &0.3822    &0.3915    &0.4150    &0.4320    &0.4260    &0.4642    &0.4648    &0.4826 \\
%&   MCFS          &0.x    &0.2961    &0.3045    &0.3249    &0.3517    &0.3850    &0.4009    &0.4486    &0.4523    &0.4637 \\
%&   FSASL15       &0.x    &0.2424    &0.2924    &0.3234    &0.3483    &0.3763    &0.3941    &0.3926    &0.4115    &0.4535 \\ %alpha=1
%&   LASSO1        &0.x    &0.2503    &0.2503    &0.2506    &0.2507    &0.2507    &0.2506    &0.2506    &0.2506    &0.2506 \\
%&   L20ALM     &0.x    &0.2356    &0.3132    &0.3302    &0.3483    &0.3336    &0.4459    &0.4179    &0.4266    &0.4705\\%巨慢
%&   Our\_L1             &0.x    &0.3343    &0.4051    &0.4266    &0.4792    &0.5064    &0.5397    &0.5216    &0.5333    &0.5719 \\
%&   Our\_L1\_center      &0.x    &0.3343    &0.4138    &0.4372    &0.4663    &0.5310    &0.5915    &0.5484    &0.5711    &0.5919 \\
%&   Our        &0.x    &0.3604    &0.4826    &0.5023    &0.5064    &0.5450    &0.5261    &0.5753    &0.5828    &0.5930 \\
%&   Our\_nor\_con    &0.x    &0.2995    &0.3563    &0.3918    &0.4459    &0.4750    &0.4773    &0.5378    &0.6097    &0.5934   \\
%&   center\_semantic   &0.x    &0.3014    &0.3737    &0.4257    &0.4007    &0.4357    &0.4650    &0.4766    &0.4879    &0.5034 \\
%&   center\_binary      &0.x    &0.2470    &0.2765    &0.3056    &0.3498    &0.3238    &0.3952    &0.3865    &0.4115    &0.4138 \\
%&   Our\_L1\_s\_binary       &0.x    &0.3487    &0.3336    &0.4603    &0.4576    &0.4864    &0.4868    &0.4902    &0.5291    &0.5238 \\
%&   LASSO0.1        &0.x    &0.2470    &0.2765    &0.3056    &0.3498    &0.3238    &0.3952    &0.3865    &0.4115    &0.4138    \\
%&   Our\_L1\_center\_b        &0.x    &0.3487    &0.3336    &0.4603    &0.4576    &0.4864    &0.4868    &0.5008    &0.5291    &0.5238    \\
%\hline
%\multirow{7}{*}{NMI} &
%    Random          &0.0416    &0.0578    &0.0732    &0.0814    &0.0957    &0.1044    &0.1224    &0.1376    &0.1423    &0.1563 \\
%%&   LapScore      &0.x    &0.1822    &0.2004    &0.2104    &0.2021    &0.2613    &0.2842    &0.2842    &0.2930    &0.2946  \\
%&   MCFS          &0.x    &0.2780    &0.2881    &0.2899    &0.3428    &0.3800    &0.4062    &0.4309    &0.4399    &0.4550 \\
%&   FSASL15        &0.x    &0.1420    &0.2124    &0.2431    &0.2746    &0.2921    &0.3275    &0.3230    &0.3494    &0.3893 \\
%&   LASSO1        &0.x    &0.00027    &0.00029    &0.00058    &0.00063    &0.00070    &0.00057    &0.00066    &0.00076    &0.00071    \\
%&   L20ALM     &0.x    &0.1564    &0.2549    &0.2461    &0.2439    &0.2447    &0.3701    &0.3801    &0.4002    &0.4208\\%巨慢
%&   Our\_L1             &0.x    &0.3219    &0.3655    &0.4058    &0.4239    &0.4609    &0.4772    &0.4933    &0.4993    &0.5326 \\
%&   Our\_L1\_center      &0.x    &0.3219    &0.3832    &0.4031    &0.4328    &0.4735    &0.5105    &0.5253    &0.5294    &0.5571 \\
%&   Our        &0.x    &0.x    &0.4093    &0.4560    &0.4692    &0.5104    &0.5320    &0.5689    &0.5823    &0.5918 \\
%&   Our\_nor\_con    &0.x    &0.2715    &0.3088    &0.3759    &0.4039    &0.4459    &0.4597    &0.5108    &0.5627    &0.5793   \\
%&   center\_semantic   &0.x    &0.2791    &0.3117    &0.3665    &0.3688    &0.4159    &0.4277    &0.4546    &0.4864    &0.4933 \\
%&   center\_binary      &0.x    &0.1546    &0.1845    &0.2470    &0.2883    &0.2788    &0.3693    &0.3663    &0.4026    &0.4094 \\
%&   Our\_L1\_s\_binary       &0.x    &0.3178    &0.3499    &0.4354    &0.4158    &0.4605    &0.4578    &0.4667    &0.4772    &0.4840 \\
%&   LASSO0.1        &0.x    &0.1546    &0.1845    &0.2470    &0.2883    &0.2788    &0.3693    &0.3663    &0.4026    &0.4094    \\
%&   Our\_L1\_center\_b        &0.x    &0.3178    &0.3499    &0.4354    &0.4158    &0.4605    &0.4578    &0.4685    &0.4772    &0.4840    \\
%\hline
%\end{tabular}
%\label{tab_ndcg_results}
%\end{table*}


%\begin{table*}[htb]
%\caption{Clustering results on inverse\_SUN dataset.}
%\centering % used for centering table
%\begin{tabular}{l|l|rrrrrrrrrr}
%\hline
%    &Method & 5 & 10 & 15 & 20 & 25 &30 &35 &40 &45 &50  \\
%\hline
%\multirow{7}{*}{ACC} &
%    Random          &0.0613    &0.0728    &0.0800    &0.0838    &0.0881    &0.0906    &0.0930    &0.0956    &0.0987    &0.1006 \\
%&   MCFS          &0.x    &0.2961    &0.3045    &0.3249    &0.3517    &0.3850    &0.4009    &0.4486    &0.4523    &0.4637 \\
%&   FSASL15       &0.x    &0.2424    &0.2924    &0.3234    &0.3483    &0.3763    &0.3941    &0.3926    &0.4115    &0.4535 \\ %alpha=1
%&   LASSO1        &0.x    &0.2503    &0.2503    &0.2506    &0.2507    &0.2507    &0.2506    &0.2506    &0.2506    &0.2506 \\
%&   L20ALM     &0.x    &0.2356    &0.3132    &0.3302    &0.3483    &0.3336    &0.4459    &0.4179    &0.4266    &0.4705\\%巨慢
%&   Our\_L1             &0.x    &0.3343    &0.4051    &0.4266    &0.4792    &0.5064    &0.5397    &0.5216    &0.5333    &0.5719 \\
%&   Our\_L1\_center      &0.x    &0.3343    &0.4138    &0.4372    &0.4663    &0.5310    &0.5915    &0.5484    &0.5711    &0.5919 \\
%&   Our        &0.x    &0.3604    &0.4826    &0.5023    &0.5064    &0.5450    &0.5261    &0.5753    &0.5828    &0.5930 \\
%&   Our\_nor\_con    &0.0679    &0.0833    &0.0865    &0.0914    &0.0947    &0.0984    &0.1019    &0.1029    &0.1044    &0.1066   \\
%&   center\_semantic   &0.x    &0.3014    &0.3737    &0.4257    &0.4007    &0.4357    &0.4650    &0.4766    &0.4879    &0.5034 \\
%&   center\_binary      &0.x    &0.2470    &0.2765    &0.3056    &0.3498    &0.3238    &0.3952    &0.3865    &0.4115    &0.4138 \\
%&   Our\_L1\_s\_binary       &0.x    &0.3487    &0.3336    &0.4603    &0.4576    &0.4864    &0.4868    &0.4902    &0.5291    &0.5238 \\
%&   LASSO0.1        &0.x    &0.2470    &0.2765    &0.3056    &0.3498    &0.3238    &0.3952    &0.3865    &0.4115    &0.4138    \\
%&   Our\_L1\_center\_b        &0.x    &0.3487    &0.3336    &0.4603    &0.4576    &0.4864    &0.4868    &0.5008    &0.5291    &0.5238    \\
%\hline
%\multirow{7}{*}{NMI} &
%    Random          &0.3966    &0.4808    &0.5092    &0.5202    &0.5252    &0.5260    &0.5277    &0.5296    &0.5329    &0.5344 \\
%%&   LapScore      &0.x    &0.1822    &0.2004    &0.2104    &0.2021    &0.2613    &0.2842    &0.2842    &0.2930    &0.2946  \\
%&   MCFS          &0.x    &0.2780    &0.2881    &0.2899    &0.3428    &0.3800    &0.4062    &0.4309    &0.4399    &0.4550 \\
%&   FSASL15        &0.x    &0.1420    &0.2124    &0.2431    &0.2746    &0.2921    &0.3275    &0.3230    &0.3494    &0.3893 \\
%&   LASSO1        &0.x    &0.00027    &0.00029    &0.00058    &0.00063    &0.00070    &0.00057    &0.00066    &0.00076    &0.00071    \\
%&   L20ALM     &0.x    &0.1564    &0.2549    &0.2461    &0.2439    &0.2447    &0.3701    &0.3801    &0.4002    &0.4208\\%巨慢
%&   Our\_L1             &0.x    &0.3219    &0.3655    &0.4058    &0.4239    &0.4609    &0.4772    &0.4933    &0.4993    &0.5326 \\
%&   Our\_L1\_center      &0.x    &0.3219    &0.3832    &0.4031    &0.4328    &0.4735    &0.5105    &0.5253    &0.5294    &0.5571 \\
%&   Our        &0.x    &0.x    &0.4093    &0.4560    &0.4692    &0.5104    &0.5320    &0.5689    &0.5823    &0.5918 \\
%&   Our\_nor\_con    &0.4626    &0.5297    &0.5298    &0.5350    &0.5376    &0.5403    &0.5419    &0.5431    &0.5433    &0.5419   \\
%&   center\_semantic   &0.x    &0.2791    &0.3117    &0.3665    &0.3688    &0.4159    &0.4277    &0.4546    &0.4864    &0.4933 \\
%&   center\_binary      &0.x    &0.1546    &0.1845    &0.2470    &0.2883    &0.2788    &0.3693    &0.3663    &0.4026    &0.4094 \\
%&   Our\_L1\_s\_binary       &0.x    &0.3178    &0.3499    &0.4354    &0.4158    &0.4605    &0.4578    &0.4667    &0.4772    &0.4840 \\
%&   LASSO0.1        &0.x    &0.1546    &0.1845    &0.2470    &0.2883    &0.2788    &0.3693    &0.3663    &0.4026    &0.4094    \\
%&   Our\_L1\_center\_b        &0.x    &0.3178    &0.3499    &0.4354    &0.4158    &0.4605    &0.4578    &0.4685    &0.4772    &0.4840    \\
%\hline
%\end{tabular}
%\label{tab_ndcg_results}
%\end{table*}
%
%
%\begin{table*}[htb]
%\caption{Clustering results on inverse\_aPY dataset.}
%\centering % used for centering table
%\begin{tabular}{l|l|rrrrrrrrrr}
%\hline
%    &Method & 5 & 10 & 15 & 20 & 25 &30 &35 &40 &45 &50  \\
%\hline
%\multirow{7}{*}{ACC} &
%    Random          &0.1889    &0.1639    &0.1592    &0.1503    &0.1544    &0.1560    &0.1533    &0.1564    &0.1594    &0.1641 \\
%&   MCFS          &0.x    &0.2961    &0.3045    &0.3249    &0.3517    &0.3850    &0.4009    &0.4486    &0.4523    &0.4637 \\
%&   FSASL15       &0.x    &0.2424    &0.2924    &0.3234    &0.3483    &0.3763    &0.3941    &0.3926    &0.4115    &0.4535 \\ %alpha=1
%&   LASSO1        &0.x    &0.2503    &0.2503    &0.2506    &0.2507    &0.2507    &0.2506    &0.2506    &0.2506    &0.2506 \\
%&   L20ALM     &0.x    &0.x    &0.3132    &0.3302    &0.3483    &0.3336    &0.4459    &0.4179    &0.4266    &0.4705\\%巨慢
%&   Our\_L1             &0.x    &0.3343    &0.4051    &0.4266    &0.4792    &0.5064    &0.5397    &0.5216    &0.5333    &0.5719 \\
%&   Our\_L1\_center      &0.x    &0.3343    &0.4138    &0.4372    &0.4663    &0.5310    &0.5915    &0.5484    &0.5711    &0.5919 \\
%&   Our        &0.x    &0.3604    &0.4826    &0.5023    &0.5064    &0.5450    &0.5261    &0.5753    &0.5828    &0.5930 \\
%&   Our\_nor\_con    &0.x    &0.0833    &0.0865    &0.0914    &0.0947    &0.0984    &0.1019    &0.1029    &0.1044    &0.1066   \\
%&   center\_semantic   &0.x    &0.3014    &0.3737    &0.4257    &0.4007    &0.4357    &0.4650    &0.4766    &0.4879    &0.5034 \\
%&   center\_binary      &0.x    &0.2470    &0.2765    &0.3056    &0.3498    &0.3238    &0.3952    &0.3865    &0.4115    &0.4138 \\
%&   Our\_L1\_s\_binary       &0.x    &0.3487    &0.3336    &0.4603    &0.4576    &0.4864    &0.4868    &0.4902    &0.5291    &0.5238 \\
%&   LASSO0.1        &0.x    &0.2470    &0.2765    &0.3056    &0.3498    &0.3238    &0.3952    &0.3865    &0.4115    &0.4138    \\
%&   Our\_L1\_center\_b        &0.x    &0.3487    &0.3336    &0.4603    &0.4576    &0.4864    &0.4868    &0.5008    &0.5291    &0.5238    \\
%\hline
%\multirow{7}{*}{NMI} &
%    Random          &0.0659    &0.0847    &0.0973    &0.1008    &0.1079    &0.1150    &0.1179    &0.1239    &0.1288    &0.1365 \\
%%&   LapScore      &0.x    &0.1822    &0.2004    &0.2104    &0.2021    &0.2613    &0.2842    &0.2842    &0.2930    &0.2946  \\
%&   MCFS          &0.x    &0.2780    &0.2881    &0.2899    &0.3428    &0.3800    &0.4062    &0.4309    &0.4399    &0.4550 \\
%&   FSASL15        &0.x    &0.1420    &0.2124    &0.2431    &0.2746    &0.2921    &0.3275    &0.3230    &0.3494    &0.3893 \\
%&   LASSO1        &0.x    &0.00027    &0.00029    &0.00058    &0.00063    &0.00070    &0.00057    &0.00066    &0.00076    &0.00071    \\
%&   L20ALM     &0.x    &0.1564    &0.2549    &0.2461    &0.2439    &0.2447    &0.3701    &0.3801    &0.4002    &0.4208\\%巨慢
%&   Our\_L1             &0.x    &0.3219    &0.3655    &0.4058    &0.4239    &0.4609    &0.4772    &0.4933    &0.4993    &0.5326 \\
%&   Our\_L1\_center      &0.x    &0.3219    &0.3832    &0.4031    &0.4328    &0.4735    &0.5105    &0.5253    &0.5294    &0.5571 \\
%&   Our        &0.x    &0.x    &0.4093    &0.4560    &0.4692    &0.5104    &0.5320    &0.5689    &0.5823    &0.5918 \\
%&   Our\_nor\_con    &0.x    &0.5297    &0.5298    &0.5350    &0.5376    &0.5403    &0.5419    &0.5431    &0.5433    &0.5419   \\
%&   center\_semantic   &0.x    &0.2791    &0.3117    &0.3665    &0.3688    &0.4159    &0.4277    &0.4546    &0.4864    &0.4933 \\
%&   center\_binary      &0.x    &0.1546    &0.1845    &0.2470    &0.2883    &0.2788    &0.3693    &0.3663    &0.4026    &0.4094 \\
%&   Our\_L1\_s\_binary       &0.x    &0.3178    &0.3499    &0.4354    &0.4158    &0.4605    &0.4578    &0.4667    &0.4772    &0.4840 \\
%&   LASSO0.1        &0.x    &0.1546    &0.1845    &0.2470    &0.2883    &0.2788    &0.3693    &0.3663    &0.4026    &0.4094    \\
%&   Our\_L1\_center\_b        &0.x    &0.3178    &0.3499    &0.4354    &0.4158    &0.4605    &0.4578    &0.4685    &0.4772    &0.4840    \\
%\hline
%\end{tabular}
%\label{tab_ndcg_results}
%\end{table*}

%\begin{table*}[htb]
%\caption{Clustering results on aPY\_deep10 dataset.}
%\centering % used for centering table
%\begin{tabular}{l|l|rrrrrrrrrr}
%\hline
%    &Method & 5 & 10 & 15 & 20 & 25 &30 &35 &40 &45 &50  \\
%\hline
%\multirow{7}{*}{ACC} &
%    Random          &0.2200    &0.2606    &0.2889    &0.3163    &0.3448    &0.3656    &0.3917    &0.4109    &0.4345    &0.4519 \\
%%&   LapScore      &x    &0.2150    &0.2100    &0.2100    &0.2050    &0.2450    &0.2800    &0.2800    &0.2950    &0.2750  \\
%&   MCFS          &0.2315    &0.2961    &0.3045    &0.3249    &0.3517    &0.3850    &0.4009    &0.4486    &0.4523    &0.4637 \\
%&   FSASL15       &0.2008    &0.2424    &0.2924    &0.3234    &0.3483    &0.3763    &0.3941    &0.3926    &0.4115    &0.4535 \\ %alpha=1
%&   LASSO        &0.2470    &0.3056    &0.3238    &0.3865    &0.4138    &0.4414    &0.5961    &0.6127    &0.6127    &0.6388    \\
%&   L20ALM     &0.2068    &0.2356    &0.3132    &0.3302    &0.3483    &0.3336    &0.4459    &0.4179    &0.4266    &0.4705\\%巨慢
%&   Our        &0.2992    &0.3604    &0.4826    &0.5023    &0.5064    &0.5450    &0.5261    &0.5753    &0.5828    &0.5930 \\
%&   Our\_nor\_con    &0.2995    &0.3918    &0.4750    &0.5378    &0.5934    &0.6252    &0.6441    &0.6600    &0.6759    &0.6812   \\ %lasso_con
%&   Our\_snor\_con    &0.3113    &0.3290    &0.4020    &0.4576    &0.5148    &0.5136    &0.5234    &0.6010    &0.6023    &0.6547   \\ %lasso_con
%&   Our\_nor\_con\_R    &0.2697    &0.2995    &0.3563    &0.3918    &0.4459    &0.4750    &0.4773    &0.5378    &0.6097    &0.5934   \\
%&   center\_semantic   &0.2254    &0.3014    &0.3737    &0.4257    &0.4007    &0.4357    &0.4650    &0.4766    &0.4879    &0.5034 \\
%&   center\_binary      &0.2144    &0.2470    &0.2765    &0.3056    &0.3498    &0.3238    &0.3952    &0.3865    &0.4115    &0.4138 \\
%\hline
%\multirow{7}{*}{NMI} &
%    Random          &0.1418    &0.1897    &0.2193    &0.2467    &0.2746    &0.3003    &0.3265    &0.3484    &0.3725    &0.3950 \\
%%&   LapScore      &0.x    &0.1822    &0.2004    &0.2104    &0.2021    &0.2613    &0.2842    &0.2842    &0.2930    &0.2946  \\
%&   MCFS          &0.1839    &0.2780    &0.2881    &0.2899    &0.3428    &0.3800    &0.4062    &0.4309    &0.4399    &0.4550 \\
%&   FSASL15        &0.1165    &0.1420    &0.2124    &0.2431    &0.2746    &0.2921    &0.3275    &0.3230    &0.3494    &0.3893 \\
%&   LASSO        &0.1546    &0.2470    &0.2788    &0.3663    &0.4094    &0.4905    &0.5536    &0.6034    &0.6210    &0.6451    \\
%&   L20ALM     &0.1172    &0.1564    &0.2549    &0.2461    &0.2439    &0.2447    &0.3701    &0.3801    &0.4002    &0.4208\\%巨慢
%&   Our        &0.2354    &0.2921    &0.4093    &0.4560    &0.4692    &0.5104    &0.5320    &0.5689    &0.5823    &0.5918 \\
%&   Our\_nor\_con    &0.2715    &0.3759    &0.4459    &0.5108    &0.5793    &0.6135    &0.6356    &0.6522    &0.6702    &0.6744   \\ %lasso_con
%&   Our\_snor\_con    &0.2514    &0.3072    &0.3840    &0.4537    &0.5149    &0.5341    &0.5534    &0.5970    &0.6202    &0.6513   \\ %lasso_con
%&   Our\_nor\_con\_R    &0.2518    &0.2715    &0.3088    &0.3759    &0.4039    &0.4459    &0.4597    &0.5108    &0.5627    &0.5793   \\
%&   center\_semantic   &0.1566    &0.2791    &0.3117    &0.3665    &0.3688    &0.4159    &0.4277    &0.4546    &0.4864    &0.4933 \\
%&   center\_binary      &0.1312    &0.1546    &0.1845    &0.2470    &0.2883    &0.2788    &0.3693    &0.3663    &0.4026    &0.4094 \\
%\hline
%\end{tabular}
%\label{tab_ndcg_results}
%\end{table*}




